GroupCast: Preference-Aware Cooperative Video Streaming with Scalable Video Coding

In this paper, we propose a preference-aware cooperative video streaming system for videos encoded using Scalable Video Coding (SVC) where all the collaborating users are interested in watching a video together on a shared screen. However, each user's willingness to cooperate is subject to her own constraints such as user data plans and/or energy consumption. Using SVC, each layer of every chunk can be fetched through any of the cooperating users. We formulate the problem of finding the optimal quality decisions and fetching policy of the SVC layers of video chunks subject to the available bandwidth, chunk deadlines, and cooperation willingness of the different users as an optimization problem. The objective is to optimize a QoE metric that maintains a trade-off between maximizing the playback rate of every chunk while ensuring fairness among all chunks for the minimum skip/stall duration without violating any of the imposed constraints. We propose an offline algorithm to solve the non-convex optimization problem when the bandwidth prediction is non-causally known. This algorithm has a run-time complexity that is polynomial in the video length and the number of cooperating users. Furthermore, we propose an online version of the algorithm for more practical scenarios where erroneous bandwidth prediction for a short window is used. Real implementation with android devices using SVC encoded video on public bandwidth traces' dataset reveals the robustness and performance of the proposed algorithm and shows that the algorithm significantly outperforms round robin based mechanisms in terms of avoiding skips/stalls and fetching video chunks at their highest quality possible.

==> algorithm.tex <==


\section{Multi-Path Video Streaming without preference}
\label{sec:alg}

In this section, we will describe the algorithms for adaptively streaming SVC videos over multi-path.  We consider two scenarios: the skip based streaming and the no-skip based streaming. For the skip based streaming, the video is played with an initial start-up, (\textit{i.e.,} buffering) delay $s$ and there is a playback deadline for each of the chunks where chunk $i$ need to be downloaded by time $deadline(i)$. Chunks not received by their respective deadlines are skipped. For the no-skip based streaming, it also has a start-up delay. However, if a chunk cannot be downloaded by its deadline, it will not be skipped. Instead, a stall (\textit{i.e.,} re-buffering) will occur, \textit{i.e.,} the video will pause until the chunk is fully downloaded.
In both scenarios, the goal of the scheduling algorithm is to determine up to which layer we need to fetch for each chunk (except for those skipped), such that  the number of stalls or skipped chunks is minimized as the first priority and the overall playback bitrate is maximized as the next priority. Further, we need to determine which of the two paths to use to fetch each layer of each chunk that is decided to be downloaded.

%make fine grained decision per layer in order to find over which chunk should it be fetched such that the objective (QoE) is maximized} %Further, use of one of the link will be penalized, modeling the scenario that the cellular link is expensive.


\input{problem}


\input{hardness}
%\feng{Also need to discuss why designing the algorithm for SVC is challenging.}
%\vspace{-.1in}
\input{skipperfect}
\input{optimal}
\input{algorithm_pref}
%\input{skipperfect_E}
%\vspace{-.1in}
\input{skipwindow}

%\vspace{-.1in}
%\input{largesmall}
%\vspace{-.1in}
\input{noskip}



==> algorithm_pref.tex <==
\subsubsection{Avoide Skips Cooperative SVC }\label{sec:pref}

In this section, we consider that users (links) $1$ to $u^\prime$ have unlimited plan and can contribute as much as their bandwidth profiles allow, but users from $u^\prime+1$ to $U$ can only help avoid skips due to their limited plans.

First the No Preference Cooperative SVC Algorithm (No-Pref SVC) is run considering the base layers only (all chunks are fetched at base layer quality) to initially find if all links are equally likely used which chunks can be fetched and which chunks must be skipped due to the insufficient bandwidth using all links (line 1).

Once the base layer sizes decisions are made, the algorithm calls re-runs No-Pref SVC for base layers again but considers only the links from $1$ to $u^\prime$ and chunks that were decided to be fetched over the links $u^\prime$ to $U$. The No-Pref SVC is re-run with the objective of checking the possibility of moving every layer was decided to be fetched in any of the links $u^\prime+1$ to $U$ to the $1$ to $u^\prime$ as far as it can be fetched before its deadline. It will start from the last chunk was decided to be fetched over any of the links $u^\prime+1$ to $U$ and checks the possibility of moving it to any link from $1$ to $u^\prime$, the link that maximizes the residual bandwidth among the links $1$ to $u^\prime$ will be assigned this layer to fetch.

Finally, No-Pref SVC Algorithm continue for the next layers but with considering only the users (links) $1$ to $u^\prime$ with their remaining bandwidths after all possible base layers were fetched. 


%Move algorithm (algorithm x) which starts another backward scan using the remaining bandwidth of the links $1$ to $u^\prime$ but with the objective of checking the possibility of moving every layer was decided to be fetched in any of the links $u^\prime+1$ to $U$ to the $1$ to $u^\prime$ as far as it can be fetched before its deadline. Move algorithm finds the last index layer fetched over any of the links $u^\prime+1$ to $U$ and checks the possibility of moving it to any link from $1$ to $u^\prime$, the link that maximizes the residual bandwidth among the links $1$ to $u^\prime$ will be assigned this layer to fetch.

%Finally, No-Pref SVC Algorithm continue for the next layers but with considering only the users (links) $1$ to $u^\prime$ with their remaining bandwidths after all possible base layers were fetched. 



\begin{figure}
	\vspace{-.1in}
	\begin{minipage}{\linewidth}
		\begin{algorithm}[H]
			\small
			\begin{algorithmic}[1]
				\STATE Run No-Pref SVC algorithm for Base layers only $n=0$
				\STATE Run No-Pref SVC algorithm for Base layers ($n=0$), consider links $1$ to $u^\prime$ consider only chunks fetched over any of the links $u^\prime$ to $U$. 
				%\STATE [B,I]=Move($C$, $\mathbf{B}^{(k)}$, $\mathbf{Y}$, $I^{(u)}_n$, $k=1,...,U$, $n=0, \cdots, m$)
				\STATE Run No-Pref SVC algorithm for all layers. i.e $n=1$ to $N$ and links $1$ to $u^\prime$
			\end{algorithmic}
			\caption{Offline Avoid-Skips-SVC Algorithm }
			\label{pref-algo}
		\end{algorithm}
	\end{minipage}
	\vspace{-.2in}
\end{figure}

\if 0
\begin{figure}
	\vspace{-.1in}
	\begin{minipage}{\linewidth}
		\begin{algorithm}[H]
			\small
			\begin{algorithmic}[1]
				\STATE Obtain $a_i\le m$, which is the layer index till which chunk $i$ must be fetched based on the output of Step 1 of Algorithm \ref{pref-algo} for all $i=1, \cdots, C$.
				\STATE Initialize $R=0$, $BW = sum(B^{(2)}(1:s))$
				\FOR{each chunk $i = 1, \cdots, C$}
				 \FOR{each layer $n = 0, \cdots, a_i$ }
				 \IF{ $r_n<BW$ (chunk $i$ layer $n$ can be fetched by  link $2$)	}
				\STATE $BW=BW-r_n$
				\ELSE
				\STATE $R=R+r_n$
				\ENDIF
				\ENDFOR
				\STATE $BW = BW + sum(B^{(2)}((i-1)L+s+1: i L+s))$
				\ENDFOR
				\IF{$R>0$}
				\STATE Initialize $LEFT=R$ 
				\FOR{each chunk $i = 0, \cdots, C$}
				\IF{$B^{(1)}(i)<LEFT$}
				\STATE $LEFT = LEFT- B^{(1)}(i)$
				\ELSE
				\STATE $B^{(1)}(i)=LEFT$
				\STATE $LEFT = 0$
				\ENDIF
				\ENDFOR
				\ENDIF
			%	\STATE Output $B^{(1)}$, which is the input link $1$ bandwidth profile, which is zeroed after the cumulative profile reaches $R$. 
			\end{algorithmic}
			\caption{Link1-Save }
			\label{Link1-Save }
		\end{algorithm}
	\end{minipage}
	\vspace{-.2in}
\end{figure}
\fi


\subsubsection{general Preference Algorithm}\label{sec:pref}

In this section, we consider that users (links) $1$ to $u^\prime$ have unlimited plan and can contribute as much as their bandwidth profiles allow, but users from $u^\prime+1$ to $U$ have different preferences. For example, some of them can contribute up to the $n$th enhancement layer, and some others can only help avoid skips due to their limited plans.


Therefore, the No-Pref SVC algorithm is modified as follows:  First the No Preference Cooperative SVC Algorithm (No-Pref SVC) is run considering the lowest layer all links agreed to fetch up to it, Let's denote that layer by $m$th layer. No-Pref SVC is re-run again but after excluding the links that can't contribute any more, and consider only layers fetched over those links with an objective of finding the possibility of moving them to other links. The algorithm starts from the highest layer of the last chunk fetched over any of these links, and check the possibility of moving it to any of the other links the same way described in No-Pref SVC algorithm. The same process repeats, so the next run considers up to the lowest layer that all remaining links agreed on fetching it, then the possibility of moving all layers fetched at lower priority links to higher priority links is checked the same way. 
Finally, No-Pref SVC Algorithm ends considering only the users (links) $1$ to $u^\prime$ with their remaining bandwidths after all possible lower layers were fetched. 


%Move algorithm (algorithm x) which starts another backward scan using the remaining bandwidth of the links $1$ to $u^\prime$ but with the objective of checking the possibility of moving every layer was decided to be fetched in any of the links $u^\prime+1$ to $U$ to the $1$ to $u^\prime$ as far as it can be fetched before its deadline. Move algorithm finds the last index layer fetched over any of the links $u^\prime+1$ to $U$ and checks the possibility of moving it to any link from $1$ to $u^\prime$, the link that maximizes the residual bandwidth among the links $1$ to $u^\prime$ will be assigned this layer to fetch.

%Finally, No-Pref SVC Algorithm continue for the next layers but with considering only the users (links) $1$ to $u^\prime$ with their remaining bandwidths after all possible base layers were fetched. 

\if 0

\begin{figure}
	\vspace{-.1in}
	\begin{minipage}{\linewidth}
		\begin{algorithm}[H]
			\small
			\begin{algorithmic}[1]
				\STATE Run No-Pref SVC algorithm for Base layers only $n=0,...,m$
				\STATE Run No-Pref SVC algorithm for Base layers ($n=0$), consider links $1$ to $u^\prime$ consider only chunks fetched over any of the links $u^\prime$ to $U$. 
				%\STATE [B,I]=Move($C$, $\mathbf{B}^{(k)}$, $\mathbf{Y}$, $I^{(u)}_n$, $k=1,...,U$, $n=0, \cdots, m$)
				\STATE Run No-Pref SVC algorithm for all layers. i.e $n=1$ to $N$ and links $1$ to $u^\prime$
			\end{algorithmic}
			\caption{Offline Avoid-Skips-SVC Algorithm }
			\label{pref-algo}
		\end{algorithm}
	\end{minipage}
	\vspace{-.2in}
\end{figure}
\fi



==> aviodSkipsAlgo.tex <==
\if 0
Algorithm \ref{algo:mpsvc}. The algorithm first divides the users to sets, users with equal weight are belong to the same set. Let's denote the number of the sets by $M$. Every set $U_m, m=1,...,M$ will have $|U_m|$ number of users. $U_1$ is the set that contains the users with the highest weight, and $U_M$ is the set that contains the users with the lowest weight. 

The algorithm initially finds the cumulative bandwidth of every second $j$ and user $k$ ($r_m^{(k)(j)}$), line 4). Then, it makes the decisions for the base layer, \ie which chunks to be skipped, and which to be fetched. Moreover, the algorithm decides which user (link) will be used to fetch the base layer of every fetched chunk. If there is a set $U_m$ such that $\lambda_0 < \frac{1}{w_u}, \forall u \in U_m$, that set will not be considered since the cost of using any user's link in this set is outweighing the utility that can be achieved. The algorithm starts by performing backward scan considering only the users of the set $U_1$ (the set that contains the users with the highest weight). For example, if there is a user or more with an infinite weight ($w_u=\infty$), those users will belong to the set $U_1$. The backward scan starts from the deadline of the last chunk (line 7) and checks the possibility of fetching chunks according to the available bandwidth (line 10). Given the decisions of chunks $i+1, \cdots, L$, we wish to decide which of the links should chunk $i$ be fetched at, such that the objective function is maximized without violating deadline, bandwidth, and rate constraints. For all choices of links (users) at which chunk $i$ can be fetched, we compute the residual total bandwidth (sum of the bandwidths of all links) that will remain for the download of the chunks $1, \cdots, i-1$. The link choice that maximizes the residual total bandwidth is chosen to fetch chunk $i$ (Algorithm 2). Note that the algorithm is similar to  dynamic programming, where the algorithm decides the quality at which the chunks will be fetched starting from the last one. The link over which the chunk $i$ is fetched is the one that gives the maximum amount of total available bandwidth over all links before the deadline of chunk numbered $i-1$.  For example, consider that there are two links have infinite weight, and consider that  fetching the $i$-th chunk over the  link 1 results in using  $x$ amount of the bandwidth before the deadline of $i-1$-th chunk while fetching the $i$th chunk over  link 2 results in using  $y$ amount of the bandwidth before the deadline of $i-1$th chunk. Then, the first link will be chosen to fetch the chunk $i$ if $x<y$. 

If the algorithm reaches a chunk $i$ that can't be completely downloaded within its deadline over any link in this set, the algorithm will check the possibility of moving the base layers of the chunks $1$ to $i$ to the set with highest weight among the remaining sets ($U_2$). Note that since the $i$th chunk can't be fetched using any of the links in the first set ($U_1$), all the chunks $1$ to $i-1$ can't be fetched as well. If the utility that is achieving by moving the base layer of this chunk to a link in $U_2$ outweighs the cost. \ie $\lambda_0 > \frac{1}{w_u}, u \in U_2$, then running backward scan on this set of links will yield a decision of which chunks (base layers) can be fetched using this set of links and which chunk/chunks should every link fetch. The non-fetched chunks (base layer) are moved to the next set the same way. However, if we reach the point such that the remaining bandwidth is not enough to fetch a base layer of a single chunk, or we reach a set such that the cost of fetching single base layer outweighs the utility, then those chunks must be skipped $\lambda_0 < \frac{1}{w_u}$. Note that the skips are brought as early as possible since the earliest chunks are the closest to their deadlines. therefore, if there must be skips, skipping those will result in the highest utility since their partial bandwidth could be used to fetch higher layers of the future chunks. We will show later, if we consider only base layers, this algorithm is optimal. 

%One thing to note, since the algorithm starts scanning from back if a chunk $i$ can't be fetched over any of the links in the first set, all chunks from 1 to $i-1$ can't be fetched as well. Therefore, the backward algorithm will be run on 



%The algorithm performs forward scan using the link/links with the highest weight/weights. For example, if there is a link or more with infinite weights $w_u=\infty , u\in\ U^\prime$, where $U^\prime$ is subset of $U$ that contains the links with the highest weights; those links will be used in simulating fetching the layers in order (line 7). The algorithm checks the possibility of fetching chunks according to the available bandwidth (line 10, where $r^{(u)}(j)$ is the cumulative available bandwidth of the link $u$ up to the $j$th time slot). Given the decisions of chunks $1, \cdots, i-1$, we wish to decide over which of the links in $U^\prime$ should base layer of chunk $i$ be fetched. We choose the one that finishes fetching the base layer of the $i$th chunk before the chunk's deadline. If the base layer of the $i$th chunk can't be fetched before violating its deadline, the algorithm will check the possibility of moving the base layer of the first chunk ($i^\prime$) fetched over any of these links ($U^\prime$) to the next highest weight's set ($U^{\prime\prime}$). Therefore, if there is a link in ($u \in U^{\prime\prime}$) such that base layer of the $i^\prime$ chunk can be fetched before its deadline, the base layer will be considered to be fetched; otherwise, the algorithm will check the next set in the weight order. However, if the base layer of the $i$th chunk can't be fetched before its deadline over any of the links. The base layer of $i^\prime$ is skipped. Note, we skip the base layer of the $i^\prime$th chunk not the $i$th chunk, and the reason we do that, is that $i^\prime$ is closer to its deadline. Therefore, skipping it will benefit the utility more since all chunks which come in order after $i^\prime$th can benefit from this skip and might be able to fetch their higher layers. 

%Finally, whatever, was reserved  to fetch the base layer of the $i^\prime$th chunk will be considered as reserved to fetching the next one in order, so defiantly $i$th chunk can be fetched

 
 
 %\textcolor{red}{for the case when $\lambda=0$, so both links can be used without preferring  one over the other, and then we will for any value of $\lambda$.} 
 
 %which is summarized in Algorithm \ref{algo:mpsvc}. 
%our algorithm works from the lowest (i.e the base) to the highest enhancement layer, and processes each layer separately. It performs backward scans (explained below) at each layer given the decisions of the previous layers.
%\subsubsection{Efficient Quadratic-time Solution}\label{skipalgo}

%\textcolor{red}{In equal priority}, MP-SVC algorithm (Algorithm \ref{algo:mpsvc}) 


%The link over which the chunk $i$ is fetched is the one that gives the maximum amount of total available bandwidth over all links.  For example, assume that there are two links in the set of the highest weights ($U^\prime$), consider that  fetching the $i$-th chunk over the  link 1 results in using  $x$ amount of the bandwidth while fetching the $i$th chunk over  link 2 results in using  $y$ amount of the bandwidth before the deadline of $i-1$th chunk. Then, the first link will be chosen to fetch the chunk $i$ if $x<y$. 

%The backward algorithm (Algorithm 2) starts from fetching the base layer of each chunk $i$. It will then decide the link which leaves more bandwidth for remaining chunks (less than $i$) to fetch the layer using the link. Once the base layer decision is taken, the algorithm sequentially decides to fetch the enhancement layers using one of the links in a similar fashion. %in each of the links, and the one that leaves more bandwidth for the remaining chunks (chunks < $i$) will be assigned this layer to fetch.  The algorithm takes as input, the starting time slot of fetching layer $n$ of chunk $i$ on  the link $wifi/lte$ ($j_1/j_2$), the predicted bandwidth $B^{(1)}/B^{(2)}$, the cumulative predicted bandwidth $r^{(1)}/r^{(2)}$, and the chunk size $Y_n$, ad checks the possibility of fetching it over that link. If the remaining bandwidth of any of the links is less than a chunk size, then that link is excluded (lines 9-21, and 24-26). Otherwise, the algorithm compares the total bandwidth available for the remaining chunks (chunks $< i$) if the current chunk is fetched over WiFi with its value if the chunk is fetched over LTE link using the returns of the backward algorithm ($j_3/j_4$: the time slot in which chunk $i$ is fully downloaded over link $wifi/lte$, $B1/B2$: the remaining bandwidth of the link wifi/let, $r_1/r_2$: the remaining cumulative bandwidth up to $j_3/j_4$ of the link $wifi/lte$, lines 29-37), and the link that leaves more bandwidth before the deadline of $i-1$ will be assigned this layer to fetch.} %\textbf{Difficult to parse. Can you elaborate more?} \textbf{Arnob: I tried to simplify it further, but I am not sure if it is now better, plz read and let me know what you think}


%Once the base layer decision is taken, the algorithm sequentially decides to fetch the enhancement layers. %in a similar fashion.

{\bf Enhancement layer modifications}: The algorithm proceeds in a similar fashion to decide for the next higher layer and so on. However, there are two changes; first, the $n$th layer for a chunk is not fetched if its $(n-1)$th layer was not fetched (line 9, Algorithm \ref{algo:mpsvc}). Second, the algorithm considers fetching all layers that can be fetched for every chunk up to the $n$th layer and links that contribute more to the utility than the cost, \ie any link $u \in U$ such that $\lambda_n > \frac{1}{w_u} $. The algorithm starts with the set of the highest weight $U_1$, and if the $n$th layer of the $i$th chunk can't be fetched over any of these links, the algorithm needs to move one or more layers to the next set. However, the algorithm needs to move the minimum size such that the $n$th layer of the $i$th chunk is fetched (the $n$th layer itself could be the moved layer). The complexity of finding the set of the layers with minimum size that needs to be moved such that the current layer is fetched is exponential with respect to the number of the layers. Hence, the algorithm in order to approximate the solution proceeds this way: it will check the possibility of moving a layer that was decided to be fetched over a link in this set before the deadline of the current layer and has a size that is equal to the remaining size of the current layer. If there is no such a layer, a layer with minimum size that is higher than the remaining size but not by more than the size of the lowest fetched (before the deadline of the current chunk) layer will be moved. In other words, if the remaining size is $(a)$Bytes, the size of the lowest fetched layer is $(b)$ Bytes, and there is a layer such that its size is $a+b-\delta$, for $\delta > 0$, this layer will be moved to the next set. If there is no such a layer, the algorithm will move the minimum of $\floor{\frac{\text{remaining size}}{\text{size of the largest layer}}}$ and the number of the largest layer that have been fetched before the deadline of the current chunk. Then algorithm repeats the same steps for the remaining size and layers after excluding the largest size layer. Now the remaining size is smaller since some space was freed up by moving some layers to the next set.

\fi

\if 0
\begin{figure}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:}  $\mathbf{Y}=\{Y_n\forall n\}$, $L$, $s$, $C$, $\mathbf{U}=\{U_m, m=1...,M\}$, $\mathbf{B}_m^{(u)}=\{B_m^{(u)}(j)\forall j\}$, $u=1, 2,......,|U_m|$. 
				\STATE {\bf Output:} $I^{(u)}_{m,n}$, $u=1,...,|U_m|$, $m=1,...,M$, $n=0,...,N$: set containing the indices of the chunks that can have their $n$th layer fetched over link $u$.
					
    \STATE  $deadline(i)=(i-1)L+s \quad \forall i$ 
     \STATE  $r_m^{(u)}(j)=\sum_{j^\prime=1}^{j} B_m^{(u)}(j^\prime)$, $j=1,....deadline(C)$, $u=1,...., |U_m|$, $m=1,...., M$
    % \STATE $remainigLayers \leftarrow$ $\mathbf{Y}=\{Y_n\forall n\}$
    \FOR{each layer $n = 0, \cdots, N$}
      
     \STATE $j_{1}=j_{2}=....=j_{|U_{m}|}=deadline(C)$
    \FOR{$m=1:M$}
     %{\bf j not defined - need efficient loop - should be also outside $n$ loop. }
    % available bandwidth on lte connection up to time $j, \forall j$
    \FOR{$i=C:-1:1$}
    \STATE $j_k =\min(j_k, deadline(i))$, $k$
    	\IF{($n=0$ or $i \in I_{n-1}^{(1)}$ or $i \in I_{n-1}^{(2)})$}
    		\IF{$max(r_m^{(1)}(j_1),...., r_m^{(|U_{m}|)}(j_2)) \geq Y_n$ and $Y_n \neq 0$}
      			\STATE $[R_m^{(u)},B2_m^{(u)}, j2_m^{(u)}, nf_m^{(u)}] = backward(i, j_u, \{r_m^{(u)}(j)\forall j\}, \mathbf{B}_m^{(u)}, Y_n)$, $u=1, 2,...|U_m|$
      		%	\STATE $tmp^{(k)}=0$, $k=1, 2$% {\bf Anis, check $\infty$ or zero, since you will be doing max later. If not fetched and has infinite residual bandwidth, this will be chosen. }
      		%	\FOR{k=1:2}
      		%	\IF{$nf^{(k)}=0$}
      			\STATE $tmp(k)=(1-nf_m^{(u)})R_m^{(u)}(deadline(i-1))+\sum_{u^\prime=1, u^\prime \neq u}^{|U_m|} r^{(u^\prime)}(deadline(i-1))$, $u=1, 2,...|U_m|$
      		%	\ENDIF
      		%	\ENDFOR
      			\STATE $u_1=\arg\max \big(tmp^{(u)\big)}$
      			\IF { $(r^{(u_1)}(deadline(i)) \geq Y_n)$}
      				\STATE $I_n^{(u_1)}=I_n^{(u_1)} \cup i$
      				\STATE $\mathbf{B}^{(u_1)}=B2^{(u_1)}$, $j_{u_1}=j2^{(u_1)}$, $r^{(u_1)} =R^{(u_1)}$
				\STATE $Y_n=0$
      			\ENDIF
			\ELSE
			\STATE $Y=move()$
      		\ENDIF
	\ENDIF
      \ENDFOR
     \ENDFOR
     \ENDFOR
   				\end{algorithmic}
				\caption{Offline MP-SVC Algorithm }\label{algo:mpsvc}
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}

\fi

\if 0	
	\begin{figure}
		%\vspace{-.6in}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $Y, deadline, U_m, U_{m+1}, r$
					\STATE {\bf Output:} 
    \STATE {\bf Initialization:}
    \STATE $i=C$,  $nf=0$
    \IF{$r < Y_n$}
    	\STATE $nf=1$
	\ELSE
     \WHILE {($Y_n > 0$)}

            \STATE $fetched=min(B(j), Y_n)$ 
            \STATE $B(j)=B(j)-fetched$, $r(j)=r(j)-fetched$, $Y_n(i)=Y_n(i)-fetched$
	   \STATE {\bf if } {$(B(j)=0)$} {\bf then }  $j=j-1$            	
    \STATE $R=r$, $B2=B$, $j2=j$        
\ENDWHILE
\ENDIF
				\end{algorithmic}
				\caption { Move Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}
\fi




==> conclusions.tex <==
\section{Conclusions}\label{sec:concl}
%\vspace{-.1in}

This paper provides an adaptive streaming algorithm for a  video encoded with Scalable Video Coding (SVC) over multiple paths, where each layer of every chunk can be fetched from only one of the two paths. The problem for optimizing the user's quality of experience (QoE) is formulated as a combinatorial optimization problem. It is shown that this combinatorial problem can be solved optimally with a complexity that is quadratic in the video length. Further, an online algorithm is proposed where 
several challenges including  bandwidth prediction
errors are addressed. The proposed algorithms are further extended when one of the link is preferred over the other. Extensive simulations and emulations with real traces of public dataset reveal the robustness of our schemes and demonstrate their significant
performance improvement compared to other state-of-the-art multi-path algorithms.


==> emulation.tex <==
\section{Emulation Results}\label{sec:emu}

\begin{figure}
\centering
\vspace{-.2in}
\includegraphics[trim=0in 2in 0in 0in, clip,width=0.4\textwidth, height=2in]{emuSys.pdf}	
\vspace{-.3in}
 \caption{System Architecture for Emulation of MP-SVC.}
 \label{fig : emuSys}
% \vspace{.5in}
 \end{figure}


\begin{figure}
	\input{emuProfilesV2.tex}
	\vspace{-.2in}
 \caption{(a) Link 1 bandwidth profile, and (b) Link 2 bandwidth profile.}
\label{fig : emuProfiles}
\end{figure}


%\begin{figure}
%\centering
%\vspace{-.4in}
%\includegraphics[trim=0in 0in 0in 0in, clip,width=0.48\textwidth]{emuProfiles.eps}	
%\vspace{-.1in}
% \caption{(a) Link 1 bandwidth profile, and (b) Link 2 bandwidth profile.}
% \label{fig : emuProfiles}
% %\vspace{-.3in}
%\vspace{-.2in}
% \end{figure}
%

To complement our simulation results, we have built an emulation testbed, which is depicted in Fig.~\ref{fig : emuSys}. The server, and the client nodes are both running in a Linux machine with kernel version 2.6.32, 24 CPU cores, and 32MB memory. The server and client communicate with each other via the loopback interface using the default TCP variant, TCP CUBIC~\cite{ha2008cubic}. Two orthogonal links were created to emulate the behavior of the multi-path streaming. To fetch a layer of a chunk, the client sends a request for that layer to the server via one of the two links, determined by our algorithm, thus the server will send back the data packets of that chunk layer via the same link. The emulation ends when all chunks are received and played back. We record the received time, the playback time and the actual number of layers received for every chunk. To introduce bandwidth variations into the emulated experiments, we adopt \texttt{Dummynet}~\cite{dummynet} running on the client side, thus the incoming rates of the TCP packets from the server on the both links (i.e., 1 or 2) will be throttled according to the bandwidth datasets used. The bandwidths profile of the datasets for the both links are described in Section \ref{sec:eval}, from which one profile of each dataset is chosen and are depicted in Fig.~\ref{fig : emuProfiles}. 
The emulation results using these bandwidth profiles are compared with the simulation results, and the comparison is qualitatively similar for the other profiles. Thus, only the depicted profiles are used in this section.  The chosen bandwidth profiles have an overall max/mean/min values of 5.9, 1.68 and 0 Mbps for link $1$ (which has higher variance than link $2$), and 1, 0.88 and 0.65 Mbps for link $2$.
%\if 0
%\begin{figure}
%\centering
%\vspace{-.2in}
%\includegraphics[trim=0.4in 0in 0.25in 0in, clip,width=.48\textwidth]{em_vs_sim.eps}	
%\vspace{-.1in}
% \caption{Comparison of Emulation With Simulation results of MP-SVC, (a) Playback Quality CDF, and (b)  Playback Quality with time}
% \label{fig : emuVsSim}
% %\vspace{-.3in}
% \end{figure}
% \fi
 \begin{figure}
 \centering
\input{sim_vs_em_equal_skip}
\vspace{-.3in}
\caption{Simulation vs Emulation for equal priority skip based streaming (a) Quality CDF, and (b) Playback rate}
\label{fig : emuVsSim}
 \end{figure}
\begin{figure}
\centering
\input{sim_vs_em_pref_skip}
\vspace{-.3in}
\caption{Simulation vs Emulation for Link preference skip based streaming (a) Quality CDF, and (b) Playback rate}
\label{fig : emuVsSimPref}

 \end{figure}

 
For both simulation and emulation, we consider the parameters as described in Section \ref{sec:eval}. We note that the mean run time for the algorithm for a window size of 10 chunks (40 s) was 7.6 ms over a large number of runs for the different bandwidth profiles. This depicts the computational efficiency of the proposed algorithm. 

Figures \ref{fig : emuVsSim} and  \ref{fig : emuVsSimPref}  compare the playback quality of simulation and emulation for both equal priority and Link preference skip based streaming, respectively.  Figures \ref{fig : emuVsSim}-a and \ref{fig : emuVsSimPref}-a  plot the CDF of the playback quality, and Figures \ref{fig : emuVsSim}-b and  \ref{fig : emuVsSimPref}-b depict the playback bit rate in Mbps over time. From these figures, we note that the emulation results closely match the simulation results in terms of playback quality. Moreover,  the Link 1 usage achieved by emulation also matches the simulation results (not depicted in a figure). Therefore, the emulation results confirm the practicality of the proposed algorithm. 

%One more thing worth mentioning is that in the playback rate figures (Fig.~\ref{fig : emuVsSim}-b and Fig.~\ref{fig : emuVsSimPref}-b), we see that the playback rate curve starts at zero since the startup delay is 5s, so first chunk is played after 5 seconds. Moreover, as it was explained in section.~ \ref{sec:bw_err}, the first two chunks are fetched at base layer quality, and that is why we see the playback rate starts at 0.6Mbps (BL rate).

%The chosen bandwidth profiles have the first link bandwidth higher in the start, and decreases later on. This impacts the quality decisions, where the earlier chunks are fetched at higher quality which degrades later. Both the simulation and emulation results show similar drops and increases of rates. 

% are high at the beginning and runs low close to the end, the quality decisions up to the chunk numbered 200 were fetched at highest quality level for both simulation and emulation, and when the average bandwidth dropped we started to see the algorithm changing the requesting policy, and running into quality switches and skips in the same manner for both emulation and simulation.


==> hardness.tex <==
\subsection{Structure of the Proposed Problem}

The problem defined in~\S\ref{sec:problem} has integer constraints and a non-convex constraint (in \eqref{equ:c5eq1}). Integer-constrained  problems are in the class of discrete optimization \cite{nemhauser1988integer}. Some of the problems in this class are the Knapsack problem, Cutting stock problem, Bin packing problem, and Traveling salesman problem. These problems are all known to be NP hard. Very limited problems in this class of discrete optimization are known to be solvable in polynomial time, some typical examples being shortest path
trees, flows and circulations, spanning trees, matching, and matroid
problems. The well known Knapsack problem optimizes a linear function with a single linear constraint ( for integer variables), and is known to be NP hard. The optimization problem defined in this paper has multiple constraints (including non-convex constraints), and does not lie in any class of known  problems that are polynomially-time solvable to the best of our knowledge. 

We note that optimization based formulations have been proposed earlier for video streaming \cite{MPC,6115763,Ahmedin:2014:ESV:2741897.2741942,FENG2017}. However,  the optimality of these algorithms have not been considered due to integer constraints. The non-convex constraint in \eqref{equ:c5eq1} further increases the problem complexity beyond the proposed ILP formulations in \cite{6115763,Ahmedin:2014:ESV:2741897.2741942}.   In this paper, we will show that the proposed  optimization
problem can be solved optimally in polynomial time. However, the result is not for general parameters and hold when \eqref{basic_gamma_1} is  satisfied. As explained earlier, this range is meaningful to reduce the skips, and preference of lower layers to higher layers.%, and minimizing link $1$ usage  while maximizing the quality.

==> introv2.tex <==
\section{Introduction}
\label{sec:intro}
	It is common that today's to have WiFi and cellular networks exist in the same physical place at the same time. The provision of simultaneous access of the multiple interfaces significantly improves the performance of various applications, as they can leverage the bandwidths of multiple WiFi and LTE links. Video streaming is one of the major sources of  traffic in mobile networks. While its popularity is on the rise, its quality of experiences (QoE) is still often far from satisfactory. In this paper, we propose a set of efficient video streaming algorithms to improve users' QoE using multiple paths simultaneously. 



There are two popular coding techniques, Advanced Video Coding(e.g H.264/MPEG4-AVC) and Scalable Video Coding (SVC~\cite{SVC_encoding}).
In AVC, each video chunk is stored into $L$ {\em independent} encoding versions. When fetching
a chunk, 
the player's adaptation mechanism, Adaptive Bit Rate (ABR) streaming, needs to select one out of the $L$ versions based on its estimation of the network condition and the buffer capacity. 

In SVC, each chunk is encoded into ordered \emph{layers}: one \emph{base layer} (Layer 0) with the lowest playable quality, and multiple \emph{enhancement layers} (Layer $i>$0) that further improve the chunk quality based on layer $i-1$.  For decoding a chunk up to enhancement layer $i$, a player must download all layers from 0 to $i$. Thus, adaptive SVC streaming can allow playback at a lower quality if all the enhancement layers have not been fetched while ABR streaming does not allow playback if the chunk is not fully downloaded. adaptive SVC streaming has been shown to provide better adaptiveness and scalability than ABR \cite{SVCMetrics,Sanchez12}. That is why we choose SVC as the coding scheme in this paper and propose a set of streaming algorithms using SVC. 



In this paper, we assume the problem in which multiple WiFi access pints and LTE users with different LTE carriers and data plans (e.g, unlimited, 6G, etc) are interested in watching the same video in one screen, and they are willing to cooperate in order to maximize the quality of the video. However,  their cooperation is constrained to their plans. For example an LTE user with 2G data plan is willing to cooperate in order to avoid skips/stalls (fetch the base layer if other links failed to do so) but not more than that. Moreover, LTE links are less energy efficient since they are further away from their base stations; therefore, even if there is an LTE link with unlimited plan it still can be less preferred than the WiFi when energy is considered.

In this paper, we propose a cooperative video streaming system in which multiple users can come to a cooperation agreement and proceed to watch the video in single and big screen. We consider two classes of streaming algorithms: {\em skip based} and {\em no-skip based} streaming.
 The former is for real-time streaming: each chunk is associated with a deadline, chunks not received by their their deadlines are skipped. For no-skip based streaming, if a chunk cannot be received by its deadline, it will not be skipped; instead, a stall (re-buffering) will incur until it is fully received. For both scenarios, we first, theoretically formulate the cooperative video streaming with link preference for perfectly predicted bandwidths of all links as an optimization problem with the objective of maximizing the video quality and minimizing the stalls/skips simultaneously (c.f., Section 3). Even though the formulation is a non-convex optimization problem, we develop novel, practical, and efficient set of algorithms that achieves the optimal solution of the problem in a polynomial-time for some practical scenarios. Therefore, we provide theoretic upper bound for some of the very practical scenarios (c.f., Section 3), and we propose an efficient heuristic for general case. The streaming algorithm decides whether to fetch a layer of the chunk or not, and which link to use for fetching. This approach requires no change to the server side. We note that the different layers of a chunk can be fetched using different links using adaptive SVC streaming, while the entire chunk is fetched from the same link when using ABR. This flexibility helps to provide additional improvement on QoE compared to ABR-based mechanisms. As shown in Section \ref{sec:eval}, our SVC-based multi-path streaming algorithms outperform the one of the recent state-of-the-art ABR-based multi-path streaming algorithms, MSPlayer \cite{chen2016msplayer}.


 In practice, the future bandwidth cannot be perfectly predicted, but can be estimated for a smaller window ahead using a crowd-sourced method to obtain historical data \cite{Riiser12,GTube}, or harmonic mean of the past bandwidth \cite{chen2016msplayer}. The perfect prediction case forms an upper bound to the algorithm performance with imperfect prediction. Our proposed adaptive streaming algorithms incorporate this imperfect information by using the bandwidth prediction methods in \cite{Riiser12,GTube,chen2016msplayer} (these prediction methods are not perfect thus have errors) as shown in the online algorithms in Section 3 and 4. 
 
 

\if 0

{\bf Our Contributions:} The main contributions of the paper are as follows.

\BULLET We  formulate the multi-path SVC video streaming with perfect  bandwidth prediction  as an optimization problem, whose objective is to maximize the users' quality of experience (QoE). We consider two classes of streaming algorithms:  skip based and  no-skip based streaming. For both algorithms, the goal of the scheduling algorithm is to determine up to which layer we need to fetch for each chunk (except for those skipped in realtime streaming), such that the overall playback bitrate is maximized and the number of stalls or skipped chunks is minimized.  We also propose an online algorithm for the scenario where  bandwidth prediction is not perfect, \ie available for short period ahead and has errors.

\BULLET The proposed problem is a non-convex discrete optimization problem, which is NP-hard in general since there are discrete variables and  non-convex constraints. However, we develop an efficient algorithm that solves this specific problem optimally in polynomial time. Thus, we provide a class of discrete optimization problem that is solvable optimally in polynomial time under certain assumptions. 
Specifically, we solve the proposed integer-constrained problem using  an easy-to-solve bin-packing based algorithm whose complexity is quadratic in the number of chunks. %\textcolor{red}{ Therefore, we 
\BULLET We propose streaming algorithms for the case in which one of the links is preferred over the other one. Both classes of streaming algorithms:  skip based and  no-skip based streaming are considered. 

\BULLET We also propose special cases of our approach, \ie a set of single path adaptive streaming algorithms using MPTCP for all the above cases, \ie with and without preference, and skip-based or no-skip-based. These algorithms can be used on either of ABR or adaptive SVC schemes.

\BULLET  {We evaluated our algorithms using a TCP/IP test bed with real SVC encoded videos and bandwidth traces from public datasets collected from commercial  networks. The evaluation demonstrates that our approach is robust to prediction errors, and works well with a short prediction window, where we estimate the bandwidth using harmonic mean of the bandwidth values of the past few seconds. Even though our formulation considers constant bit rate (CBR) encoding rate per layer, we evaluated our formulation and algorithms using Variable Bit Rate (VBR) encoded videos against a number of adaptive streaming strategies including the multi-path version of the buffer-based approach (MP-BBA) \cite{BBA} and the prediction based algorithms such as MSPlayer~\cite{chen2016msplayer}.} 
%
The results demonstrate that our algorithm outperforms them by improving the key QoE metrics such as the playback quality, the number of layer switches, and the number of skips or stalls. For example, our skip based streaming algorithm was able to achieve average playback quality that is $25\%$, and $35\%$ higher than MP-BBA and MSPlayer respectively with lower stall/skip durations. The preference-aware adaptive streaming algorithms were compared with the preference-aware MPTCP based algorithms in \cite{han2016mp} and it is shown that the proposed algorithm obtains lower skips, higher average quality, and lower link $1$ usage thus demonstrating  improvement in all these metrics.


\fi

The rest of the paper is organized as follows. Section \ref{sec:related} discusses the related work. Section \ref{sec:alg} describes the problem formulation for multi-path streaming without preference to any link. Further, a quadratic-time algorithm is provided for this non convex problem, and is shown to be optimal. The algorithm is extended to the case with the use of MPTCP, and online scenarios. Both skip and no-skip scenarios are considered. Section \ref{sec:pref} further considers preference of one link over the other, modeling the scenario where the users wish to use less cellular content. Section \ref{sec:eval} presents the trace-driven evaluation results with comparison to the different baselines.  Sections \ref{proof_skip} and \ref{no_skip_apdx} show the optimality of the proposed algorithms for the skip-based and no-skip based streaming, respectively, when there is no link preference. Section \ref{sec:concl} concludes the paper. The optimality for the preference based streaming is considered in the Appendix. 

%The proofs of the optimality of the proposed algorithms in Section \ref{sec:alg}  are provided in the Appendix. 



==> noskip.tex <==
\subsection{No Skip Based  Streaming Algorithm}\label{no_skip}

In no-skip streaming (\textit{i.e.,} watching a pre-recorded video), when the deadline of a chunk  cannot be met,
%The main difference between the real-time and non-realtime streaming is that
rather than skipping it, the player will stall the video and continue downloading the chunk. The objective here is to maximize the average quality while minimizing the stall duration (the re-buffering time). The objective function is slightly different from equation~\eqref{equ:eq1} since we do not allow to skip the base layer. However, we skip higher layers.
For the constraints, all constraints are the same as skip based optimization problem except that we add constraint~(\ref{equ:d10eq1}) to enforce the base layer (BL) size to be equal to the BL size of the chunk (it can't be zero). %It can't take zero value, and we add a constraint to put upper bound to the startup delay. %We minimize the startup delay and later stalls such that the startup delay do not exceed a certain threshold.
We define the total stall (re-buffering) duration from the start till the play-time of chunk $i$ as $d(i)$. Therefore, the deadline of any chunk $i$ is $(i-1)L+s+d(i)$.  The objective function is thus given as $ \sum_{n=1}^{N}\gamma^n\sum_{i=1}^{C} Z_{n,i}-\mu d(C),$
where the weight for the stall duration is chosen such that $\mu \gg 1$, since users tend to care more about not running into re-buffering over better quality. 
This is a multi-objective optimization problem with quality and stalls as the two objectives, and is formulated as follows.
\begin{eqnarray}
%\hspace{-0.2in}
&maximize \Bigg(\sum_{u=1}^U\sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C}\sum_{j=1}^{dealine(C)} z_{n}^{(u)}(i,j)-\mu d(C)\Bigg)
\label{equ:eq2}
\end{eqnarray}
%\vspace{-.1in}
%\begin{align*}
%& maximize \Bigg(\sum_{n=0}^{N}\gamma^n\sum_{i=1}^{C}q(Z_{n,i})\Bigg)
%\label{equ:eq1}
%\end{align*}
subject to  \eqref{equ:c2eq11}, \eqref{equ:c3eq1}, \eqref{equ:c55eq1},  \eqref{equ:c7eq1}, 
\begin{eqnarray}
\sum_{j=1}^{(i-1)L+s+d(i)} z_n^{(2)}(i,j)+z_n^{(1)}(i,j) = Z_{n,i}\quad  \forall i,  n 
\label{equ:d2eq1}
\end{eqnarray}
%\vspace{-.1in}
\begin{equation}
\left(\sum_{j=1}^{(i-1)L+s+d(i)} z_n^{(1)}(i,j)\right)\left(\sum_{j=1}^{(i-1)L+s+d(i)} z_n^{(2)}(i,j)\right) = 0\   \forall i, n
\label{equ:d5eq1}
\end{equation}
%\vspace{-.1in}
\begin{equation}
z_n^{(k)}(i,j)= 0\   \forall \{i: (i-1)L+s+d(i) > j\}, k\in \{1,2\}
\label{equ:d6eq1}
\end{equation}
%\vspace{-.1in}
\begin{equation}
d(i) \geq d(i-1)\geq 0\   \forall i>0 \label{deq}
\end{equation}
%\vspace{-.1in}
\begin{equation}
Z_{0,i} =Y_0
\label{equ:d10eq1}
\end{equation}
\vspace{-.2in}
\begin{eqnarray}
\text{Variables:}&& z_n^{(2)}(i,j), z_n^{(1)}(i,j),  Z_{n,i}, d(i) \forall   i = 1, \cdots, C,  \nonumber \\
&& j = 1, \cdots, (C-1)L+s+d(C), n = 0, \cdots, N \nonumber
\end{eqnarray} 


We note that this problem can be solved using an algorithm similar to that for the skip-based streaming. One difference as compared to the skip version is that the first step of the no-skip algorithm is to determine the minimum stall time since that is the first priority. Therefore, the backward scan is modified as follows:
%\textbf{Did not understand. Why are you adding the stall duration needed to increase the residual bandwidth. Why are you increasing the start-up delay?} 
First, if we find a skip, the deadline of the later chunks are shifted to add the stall duration since the last chunk   has to be fetched before the sum of the deadline and the stall duration.  %in the backward scan using $deadline(C)$, if we find a skip, the deadline of the last chunk is shifted to add the stall duration needed to increase the residual bandwidth to avoid the skip ($deadline(C)=previous \quad deadline(C)+stall \quad time$. ). 
Second, we  try to avoid stalls in the middle of playing the video. Hence, if there is a stall in the middle of the video, we will increase the start-up delay by that amount\footnote{If the start-up delay is fixed, obviously, there will be stall in the middle of the playback of the video}. This will help in not having any stall in the middle of the video. Note that increasing the start-up delay will not reduce the penalty term for the duration of stalls, hence, our algorithm will still give the minimum possible duration of stalls. We are only shifting the stalls to the beginning of the video in order to provide a smooth viewing experience and increase the opportunity of fetching higher layers of later chunks. This increased opportunity for fetching higher layers  is indeed essential to prove the optimality of the proposed algorithm. 




 % for the later chunks as it minimizes the switching rate across the chunks. So, if we find any stall, we consider that the stall time is added to the startup delay, so all stalls are brought to the very start. Thus,  there will be no stalls in the middle of playback.

%We call this backward scan No-Skip backward scan algorithm. 

The rest of the algorithm is equivalent to skip version since skips are not allowed only for base layers (higher layers can be skipped). The detailed steps are given in Algorithm \ref{algo:no_skip}. The key difference in the no-skip version is that the startup delay is decided such that there will be no skips. All the lemmas and optimality theorems of skip version are applicable to no-skip version, and the detailed optimality statements are given in Section \ref{no_skip_apdx}.

%are omitted due to lack of space. %given in the Appendix. 

\begin{figure}
		%\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				
   \STATE $d(i)=0$, $\forall i$,  $deadline(i)=(i-1)L+s+d(i) \quad \forall i$ 
     \STATE  $r^{(k)}(j)=\sum_{j^\prime=1}^{j} B^{(k)}(j^\prime)$, $j=1,....deadline(C)$, $k=1, 2$, $n=0$
%    \FOR{each layer $n = 0, \cdots, N$}
     %{\bf j not defined - need efficient loop - should be also outside $n$ loop. }
    % available bandwidth on lte connection up to time $j, \forall j$
   %	 \IF{$n > 0$}
   	% 	\STATE run MP-SVC
   % 	\ELSE
   		 \STATE $j_{1}=j_{2}=deadline(C)$
    		\FOR{$i=C:-1:1$}
    		\STATE $j_k =\min(j_k, deadline(i))$, $k=1, 2$
    			\IF{$max(r^{(1)}(j_1), r^{(2)}(j_2)) < Y_n$}
				\STATE $residual=Y_n - max(r^{(1)}(j_1), r^{(2)}(j_2))$
				\STATE increase $s$ by time required to obtain the residual, $deadline(i)=(i-1)L+s+d(i) \quad \forall i$ 
				\STATE Go to line 3. 
			\ELSE
				\STATE  run Steps 11-16 of Algorithm \ref{algo:mpsvc} to determine the link to fetch chunk $i$, update residual bandwidths, and $j_k$
     % 			\ENDIF
      		
	
  %    		\ENDFOR
      	\ENDIF
     \ENDFOR
     \STATE Run Algorithm \ref{algo:mpsvc} (Steps 6-20) for each layer $n=1, \cdots, N$. 
   				\end{algorithmic}
				\caption{Offline No-Skip MP-SVC Algorithm }\label{algo:no_skip}
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}



{\bf Online No Skip MP-SVC Algorithm}: In reality, we may not be able to predict the bandwidth for the entire video upfront, and thus all the stalls cannot be moved to the start. Based on the sliding window based approach described in Section \ref{sec:bw_err}, we bring the stalls in the window $W$ to the start of the window. After this change, the rest of the algorithm does similar adaptations to the offline schedules as in Section \ref{sec:bw_err}.




%Therefore, the online algorithm brings the stalls corresponding to the next $W$ seconds to the beginning of the current re-optimization period. Moreover, \textcolor{red}{since we use harmonic mean to predict the future bandwidth, at the beginning there will be no bandwidth prediction at all}. Therefore, the algorithm starts by fetching the first two chunks over the two links at the base layer quality so the achievable throughput can be used to predicted the future bandwidth.

%The remaining is same as the online algorithm of skip version except that base layers can't be skipped.


 % No-skip is special case from skip, when the startup delay is chosen such that all base layers can be fetched (no base layer skips).


==> noskipsims.tex <==
\subsection{No-Skip Based MP-SVC Algorithm}
\label{sec:eval_noskip}
\if 0
\begin{figure*}
%\vspace{-.1in}
\centering
\begin{minipage}{.49\textwidth}
\includegraphics[trim=1.2in 0in .5in 0.5in, clip,  width=\textwidth, height=3in]{./multiPath_results/noSkip_results.eps}	
\caption{No-Skip based streaming results on Dataset1: (a) layer distribution, (b) CDF of average playback rate, and (c) CDF of re-buffering time.}
% \label{fig : noSkipComp}
%\vspace{-.3in}
%\end{figure}
\end{minipage}
\begin{minipage}{.49\textwidth}
\centering
%\begin{figure}
%\vspace{-.1in}
\includegraphics[trim=1.2in 0in .5in 0.5in, clip,  width=\textwidth, height=3in]{./multiPath_results/noSkip_results_fcc.eps}	

\caption{No-Skip based streaming results on Dataset2: (a) layer distribution, (b) CDF of average playback rate, and (c) CDF of re-buffering time.}
 \label{fig : noSkipComp2}
%\vspace{-.3in}
\end{minipage}
\end{figure*}
\fi

\begin{figure}
\vspace{-.15in}
\centering
\includegraphics[trim=1in 0in .5in 0.5in, clip,  width=.5\textwidth]{./multiPath_results/noSkip_results.eps}	
\vspace{-.7in}
\caption{No-Skip based streaming results: (a) layer distribution, (b) CDF of average playback rate, and (c) CDF of re-buffering time.}
 \label{fig : noSkipComp}
%\vspace{-.3in}
%\end{figure}
\vspace{-.2in}
\end{figure}

%{\bf mention buffer threshold}
%Since the algorithms are similar, the results are qualitatively similar to those described in Section \ref{sec:eval_skip}

In this subsection, we evaluate our proposed algorithm for the No-Skip based scenario. The initial startup delay is chosen to be the minimum of 1s and the download time of the first chunk while the other parameters are the same as in the skip-based version. The results are shown in Fig.~\ref{fig : noSkipComp}. The main difference in the no-skip version is that since there are no skips, the video may have multiple stalls. Thus, in Fig.~\ref{fig : noSkipComp}, we evaluate the duration of stalls (re-buffering time) as an additional metric. We omit the layer switching rate since the results are qualitatively similar to skip version ones. 

We first note that MPTCP-SVC in general performs better than MP-SVC in term of avoiding stalls since multipath TCP can be used which gives better flexibility as compared to obtaining a layer only on one path.  We see in Fig.~\ref{fig : noSkipComp} that the stall duration for MP-SVC is slightly higher as compared to MPTCP-SVC. The probability mass function of the qualities at which different chunks are obtained, and the  CDF of the average video playback rate results show  that the performance of MP-SVC  is close to that of  MPTCP-SVC. 

Further, MP-SVC and MPTCP-SVC significantly outperform both MP-BBA, and MPTCP-BBA in term the average playback rate. They are about $38\%$, and $29\%$ higher than MP-BBA and MPTCP-BBA, respectively. Even though MSPlayer achieves the highest average playback rate, it runs into stall of duration of  more than a minute  for $50\%$ of the traces. MP-SVC and MPTCP-SVC  achieve low number of stalls, no stalls for about $80\%$ of the traces (similar to offline results), and less than $30s$ and $7$s for $90\%$ of the traces, respectively. %Moreover, the stall duration of MP-SVC and MPTCP-SVC can be reduced further if $B_{min}$ is increased (for the current simulation, $B_{min}=0$). 
 Thus, MP-SVC and MPTCP-SVC achieve a better tradeoff between the average playback rate and stall durations. 

%We see how MP-SVC, and MPTCP-SVC trade-off high average rate with low number of stalls. Without setting lower buffer threshold, they achieve low number of stalls,  less than $20s$ and $7$s for $99\%$ of the traces respectively. This stall duration could have been reduced with a cost of lower playback rate if we set a lower buffer threshold, so if the buffer runs bellow that threshold, chunks are fetched at base layer. %Finally, MP-BBA and MPTCP-BBA run into the lowest number of stalls but the cost is achieving significantly lower average playback rate with compare to MP-SVC and MPTCP-SVC.

%The only difference of the structure of the figures with compare to skip version is that we have replaced the layer switching rate subplot with stall (re-buffering time) CDF plot Fig.~\ref{fig : noSkipComp}-c and Fig.~\ref{fig : noSkipComp2}-c. We omit the layer switching rate because the results are very similar to skip version case.. The key observations from Fig.~\ref{fig : noSkipComp} and Fig.~\ref{fig : noSkipComp2} are:

%

%\begin{itemize}
%\item MP-SVC neither require any kernel modification nor network worries of blocking the packets, and yet achieve similar results as MPTCP-SVC. We clearly see that the results of offline MP-SVC is very close to offline MPTCP-SVC which requires MPTCP installed at both client and server. The difference is negligible. Moreover, the online MP-SVC is also very close to online MPTCP-SVC, and both are the closest to the offline MPTCP-SVC which is the best that can be achievable. 
%\item No-Skip results confirms the skip based results in stating that the MPTCP win over application layer is very negligible. We clearly see from both figures Fig.~\ref{fig : noSkipComp} and Fig.~\ref{fig : noSkipComp2} that MP-SVC and MPTCP-SVC have very similar results.

%\item MPTCP-SVC incur very negligible stall duration with compare to the offline algorithm, and MP-SVC incur little bit higher stalls in the high average regime (HSDPA dataset). However, MP-SVC could reduce this stall duration by setting a lower buffer threshold, so if the buffer occupancy is lower than that threshold, the decision is modified such that all chunks are fetched at base layer quality. In fact we did that, and we reduced the stall duration very significantly with some loss in average playback quality. {\bf: I can have results where we have lower buffer threshold, so we have one more curve}
%\item Both MP-SVC and MPTCP-SVC, achieve high average playback rate. The average playback rate is, about $33\%$, and $28\%$ higher with compare to MP-BBA, and MPTCP-BBA, respectively on HSDPA dataset, and  $30\%$, $22\%$, and $21\%$ higher with compare to MP-BBA, MPTCP-BBA, and MSPlayer on FCC dataset respectively.

%\item  Both MP-SVC and MPTCP-SVC achieve the high average and low number of skips with very competitive layer switching rate. As Fig.~\ref{fig : BComp}-c and Fig.~\ref{fig : BComp2}-c show, the CDF curve of the switching rate of MPSVC is similar to MP-BBA on HSDPA and they beat it in the FCC data because the average bandwidth of FCC dataset is low, so MP-BBA will struggle in switching between before and after the lower threshold (the startup and the linear decision regions). MP-SVC achieves very low layer switching rate and very close to the offline algorithm on FCC data with being $99\%$ of the time less than $4\%$. It is slightly higher on HSDPA dataset with being less than $20\%$ for $99\%$ of the time.

%\item MSPlayer achieve high average playback rate on high average regime (HSDPA dataset), but the cost is very expensive. It runs into so many stall durations. Fig.~\ref{fig : noSkipComp}-c shows that MSPlayer runs into about 1 minute of stall in more than $50\%$ of the traces. Moreover, it struggles with both low average playback rate and high stall duration at low average regime (FCC dataset). This clearly shows that to achieve a good trade -off between minimizing stalls and maximizing average quality both current buffer and prediction of future bandwidth are required and this what MP-SVC algorithm is doing.

%\item MP-BBA and MPTCP-BBA acheive very low re-buffering time, but the cost is significantly lower average playback rate with compare to what can theoretically be achieved.

%of over all traces. both achieve $18\%$ and $$ improvement with compare to BBA, $$ and $$ with compare to MPTCP-BBA, and $$ and $$ with compare to MSPlayer in HSDPA and FCC datasets respectively. 
%\end{itemize} 



==> optimal.tex <==
\subsection{Optimality of the No-Pref SVC}\label{optim_skip}

In this section, we prove that the proposed algorithm achieves the optimal solution of problem (\ref{equ:eq1}-\ref{equ:c7eq1}). The detailed proofs are provided in Section \ref{proof_skip}. The following result shows that the proposed algorithm minimizes the number of skips for a given layer among all the other algorithms which fetches the same quality levels up to the immediate next lower layer. %maximizes the number of chunks at least in the base layer obtained in any layer given the decisions of the previous layers. 

\begin{lemma}%{Theorem}
Given size decisions up to ($n-1$)th layer ($Z_{0,....,n-1}$), remaining bandwidth, and $deadline(i)$ for every chunk $i$, the proposed algorithm achieves the minimum number of $n$th layer skips (or obtains the maximum number of chunks at layer $n$) as compared to any feasible algorithm which fetches the same layers of every chunk up to layer $n-1$.
 \label{lem:skip1} 
\end{lemma}

Intuitively, the proposed algorithm pushes all the skips as early as possible since the earlier chunks will be closer to their deadlines, so skipping those will offer more bandwidth to the later ones, minimize the number of current layer skips, and maximize the number of candidate chunks to the next layer.
The next result demonstrates that the proposed algorithm leaves the maximum possible bandwidth before the deadline of every chunk that is a candidate (has all previous layers fetched) to the next layer.% in order to fetch its the next layer. 

\begin{lemma}%{Theorem}
Among all algorithms with the same number of $n$th layer skips, the proposed algorithm leaves the largest possible bandwidth for fetching the ($n+1$)th layer of every candidate chunk before its deadline. In other words, the proposed algorithm maximizes the resources to the higher layer among all algorithms that have same decisions up to the current layer.

%\textcolor{red}{I think this lemma needs to be re-written in a better way. We leave more bandwidth for every chunk before its deadline, so we maximize the number of candidates to the next layer.} %fetch the same number of current layer chunks . \textcolor{red}{since same number of current layer does not mean same policy up to the current layer, I think the last statement should be replaced with this one: In other words, the proposed algorithm maximizes the resources to the higher layer among all algorithms that have same decisions up to the current layer} 
%maximizes the number of candidate chunks to the next layer.%has optimal $n$th layer skip pattern
\label{lem:skip2}
\end{lemma}

Intuitively, our proposed algorithm optimizes the bandwidth resources to make more resources available for later layers. This is essential for optimality of the algorithm since the decisions for the higher layers depend on the decisions of the lower layers. Thus, if the decision of the lower layer does not help giving more resources for the higher layers, the algorithm will not be optimal.   Using Lemma \ref{lem:skip1} and Lemma \ref{lem:skip2}, the following result shows the optimality of MP-SVC algorithm in solving problem~(\ref{equ:eq1}-\ref{equ:c7eq1}).

\begin{theorem}	
Up to a given enhancement layer
 $M, M \geq 0$, if ${z_{m}^{(u)}(i,j)}^*$ is the size of the $m$th layer fetched by the $u$th use ($m \leq M$) of chunk $i$ that is found by running No-Pref-SVC algorithm, and ${z_{n}^{(u)}(i,j)}^\prime$ is a size that is found by any other feasible algorithm such that all constraints are satisfied, then the following holds when $\lambda$'s satisfy \eqref{basic_gamma_1}.%for any $0<\gamma \ll 1$. %and $\sum_{j > k}\gamma^j \sum_i Z_{j,i} \ll \gamma^k  Z_{k,1}$.
\begin{equation}
 \sum_{u=1}^U\sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C}\sum_{j=1}^{dealine(C)} {z_{n}^{(u)}(i,j)}^\prime \leq \sum_{u=1}^U\sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C}\sum_{j=1}^{dealine(C)} {z_{n}^{(u)}(i,j)}^*.
\label{thm:thm}
\end{equation}
In other words, No-Pref-SVC finds the optimal solution to the optimization problem~(\ref{equ:eq1}-\ref{equ:c7eq1}) when $\lambda$'s satisfy \eqref{basic_gamma_1}.% \textcolor{red}{and M=N}. %$0<\gamma \ll 1$.% and $\sum_{j > k}\gamma^j \sum_i Z_{j,i} \ll \gamma^k Z_{k,1}$.
\label{theorem: theorem11}
\end{theorem}
Intuitively, note that MP-SVC first fetches the lower quality level of all the chunks before fetching the next higher levels. Thus, the QoE attained is higher. It also prefers the excess bandwidth to be utilized for fetching higher quality layers of the later chunks. Finally, since MP-SVC minimizes the skips, thus, it is the optimal. 



%\textbf{Can you give any intuition why this is optimal?}


==> pref_formulation.tex <==
\section{Offline Problem Formulation For SVC Video Streaming with Preference}\label{apdx_pref}

In addition to the objectives mentioned without link preference, we further consider minimization of the link $1$ usage. In order to account for the third objective of minimization of link $1$, we consider a parameter $m\in \{0, \cdots, N\}$ indicating that the link $1$ should not be used to obtain chunks above layer $m$. This will help using link $1$ to help improve getting lower layers while not over-using it to achieve higher layers. Further, among different schemes that obtains same number of chunks till layer $m$, we wish to minimize the usage of link $1$. For $m=0$, this implies that link $1$ is only used to avoid skips and not to fetch any enhancement layers. Further, link $1$ is used only if necessary to reduce skips, when link $2$ is not sufficient to obtain the optimal number of base layer chunks. In order to account for these properties of the usage of link $1$, we subtract $D \gamma^{m+1}  \sum_{n=0}^{N}\sum_{i=1}^{C}\sum_{j=1}^{(C-1)L+s} z_n^{(1)}(i,j)$ from the objective for $\gamma$, where $D\ge 2$ satisfies

\begin{equation}
C\sum_{j=1}^{N-a} \gamma^j r_{a+j} + D \gamma^{m+1-a}r_a < r_a, \  \text{  for } a= 0, \cdots, m,  \label{basic_gamma_2}
\end{equation}
and
\begin{equation}
D  \Delta_m  > C \sum_{n=m+1}^N \gamma^{n-m-1} r_n,  \label{basic_gamma_3}
\end{equation}
where 
\begin{equation}
\Delta_m  \triangleq \min\{x: x>0, x= \sum_{i=0}^m c_i r_i, c_i \in \{-C, \cdots, C\} \}
\end{equation}


\eqref{basic_gamma_2}  is stronger than \eqref{basic_gamma_1} for $a\le m$ and for $a=m$ also gives $D<1/\gamma$. The constraint \eqref{basic_gamma_2} says that the cost of link $1$ does not constrain fetching of the lower layers, while the constraint \eqref{basic_gamma_3} wishes to limit the use of link $1$ if it does not increase the qualities of layers up to $m$. With these conditions on $D$ and $\gamma$, we will show that the above mentioned properties for the usage of link $1$ are satisfied. Overall, the multi-path SVC layer scheduling problem with the knowledge of future bandwidth information can be formulated as follows.

\begin{eqnarray}
maximize \sum_{n=0}^{N}\sum_{i=1}^{C} \Bigg(\gamma^nZ_{n,i}- D \gamma^{m+1} \sum_{j=1}^{(C-1)L+s} z_n^{(1)}(i,j)\Bigg) %- \lambda \sum_{j=1}^{deadline(C)} B(j)^{(2)}  \Bigg)
%\sum_{n=0}^{N} \lambda_n \gamma^n \sum_{i=1}^{C}\beta^i B_{n,i}^{(2)}  \Bigg)
\label{equ:eqap1}
\end{eqnarray}
%\vspace{-.1in}

subject to \eqref{equ:c2eq1}-\eqref{equ:c7eq1}
\begin{eqnarray}
\text{Variables:}&& z_n^{(2)}(i,j), z_n^{(1)}(i,j),  Z_{n,i} \ \ \  \forall   i = 1, \cdots, C, \nonumber \\&& j = 1, \cdots, (C-1)L+s, n = 0, \cdots, N \nonumber
\end{eqnarray}



We will now show that the problem formulation does not fetch any chunk using Link 1 at a layer greater than $m$. 
\begin{lemma}\label{lem_nohigher}
	None of the chunks is fetched using link $1$ for any layer greater than $m$. More precisely,  $\sum_{j=1}^{(i-1)L+s} z_n^{(1)}(i,j)=0$ for all $i\in \{1, \cdots, C\}$ and $n>m$. 
\end{lemma}
\begin{proof}
	Suppose that layer $n>m$ of chunk $i$ is fetched using link $1$. The additional utility obtained by fetching layer $n$ and higher is at most $\sum_{k=n}^{N} \gamma^k r_k$ which is lower than the loss of using Link 1 for layer $n$, which is greater than $2 \gamma^{m+1}r_n$ using \eqref{basic_gamma_1}. Thus, it is better not to fetch chunk $i$ at layers $n$ and higher if this layer is to be fetched using link $1$.
\end{proof}



Thus,  Link $1$ can only be used to fetch chunks at the layers till layer $m$. However, among any two strategies that achieve the same number of chunks at all layers till layer $m$, the proposed problem formulation will choose the one with lower Link 1 usage. This is given in the following lemma. 


\begin{lemma}\label{lem_lower}
	Among two strategies with the same number of chunks fetched at each layer from $0$ to $m$, the one that obtains lower content over link $1$ is preferred.
\end{lemma}
\begin{proof}
	For the same possible chunks till layer $m$, the minimum extra usage of link $1$ is $\Delta$. Thus, as long as the additional cost of this Link 1 usage is more than all the benefits of the layers above $m$, the cost will outweigh the benefit. Since this holds by \eqref{basic_gamma_3}, the result holds.
\end{proof}

Finally, we note that choosing link 1 for layers from $0$ to $m$ will have positive utility since $D<1/\gamma$. Finally, we need to show that if an extra chunk can be obtained at a layer $n\le m$, the above problem will not be constrained by the cost of using link $1$. This is satisfied due to \eqref{basic_gamma_2}. More formally, the following holds. 

\begin{lemma}\label{lem_lower_unc}
	Among two strategies with the same number of chunks at layer $0, \cdots, k$ for $k<m$, the strategy that obtains the largest number of chunks in layer $k+1$ achieves better objective.
\end{lemma}

Thus, we see that the utility function for the above choice of range of $(D, \gamma)$ satisfies the properties needed for the formulation. 

Even though we do not have a general algorithm that optimizes this proposed formulation for any value of $m$, the proposed algorithm MP-Pref-SVC in Section \ref{sec:pref} is optimal when $m=0$. Thus, when the objective is only to use link $1$ to avoid skips, the proposed algorithm is optimal. This is easy to see using Lemma \ref{lem_lower} that the proposed algorithm satisfies this condition. Thus, all the conditions of optimality of the additional cost function are satisfied. The key reason this does not hold for general $m$ is the greedy policy of Link1-Save algorithm in Algorithm \ref{Link1-Save }. It is not necessary for a general $m$ that this strategy will use minimum amount of link $1$. 

Finally, we note that when MPTCP can be used, the key difference is that the constraint \ref{equ:c5eq1} is removed. Thus, when partial fetching is allowed, the modification of Link1-Save  will use minimum link $1$ and thus all the conditions are satisfied for any $m$. This proves that the proposed algorithm is optimal for all values of $m$, when MPTCP can be used. We further note that the decisions made using this algorithm can be used for both SVC and AVC when MPTCP can be used.

==> pref_proofs.tex <==
\section{Proof of the optimality of Avoid-Skips GroupCast}\label{apdx_pref}
In this section, we prove that Avoid-Skips GroupCast is optimal when there are two sets each has one user. In this case there will be two users (links), and one can only help in avoiding skips. We will refer to the user 1 by link 1 and user s by link 2 in the proof. %Moreover, we prove the optimality for no maximum contribution constraint, but the results hold true when maximum contribution is imposed since that will only make the cumulative bandwidth less. 

\begin{lemma}%{Theorem}
	Avoid-Skips GroupCast  Algorithm achieves the minimum number of base layer skips.
	\label{lem:avoid_skips}
\end{lemma}
\begin{proof}
From theorem \ref{them:skip1} in section \ref{skipalgoEqual}, we know that No-Pref GroupCast algorithm achieves the minimum number of base layer skips. However, Pref GroupCast does not fetch less base layers, it only post processes the No-Pref GroupCast decisions in order to move as much as possible of base layers that have been decided to be fetched over link 2 to link 1. Therefore, the Pref GroupCast will never fetch less number of base layers than No-Pref GroupCast and that concludes the proof.
\end{proof}

\begin{lemma}\label{lem_lower}
	Among two strategies with the same number of chunks fetched at base layer, the one that obtains lower content over less preferable links is preferred.
	\label{lem:avoid_skips2}
\end{lemma}
\begin{proof}
If there are two algorithms (1 and 2) achieve the same number of base layers and algorithm 2 fetches $\Delta$ more base layers than algorithm 1 by link 2. Then, the same $\Delta$ chunks should have been fetched by link 1. Since $\lambda_0^{(1)} > \lambda_0^{(2)} $, the following holds true:
\begin{equation}
(\lambda_0^{(1)}-\lambda_0^{(2)}) \Delta >  0
\end{equation}
Which means that algorithm 1 will achieve higher objective.
\end{proof}



\begin{lemma}%{Theorem}
	Avoid Skips GroupCast Algorithm has the minimum data usage of link 2. In other words, no other algorithm can achieve less data usage for link 2 with the same number of skips as that achieved by Avoid Skips GroupCast.
	\label{lem:avoid_skips3}
\end{lemma}
\begin{proof}

Pref GroupCast re-runs No-Pref GroupCast for link 1 only (\ie use zero bandwidth of link 2) for chunks that were initially decided to be fetched by link 2 using the remaining bandwidth of link 1. From theorem \ref{them:skip1} in section \ref{skipalgoEqual}, we know that No-Pref GroupCast will fetch the maximum number of base layers. Therefore, Pref GroupCast moves the maximum number of layers from link 2 (less-preferable) to link 1 (more-preferable links). Hence minimum number of base layers will be fetched over link 2. 

\end{proof}


\begin{lemma}%{Theorem}
	Among all algorithms with the same number of base layer skips, Avoid Skips GroupCast leaves the largest possible bandwidth over link 1 for fetching the enhancement layers. In other words, the proposed algorithm maximizes the resources to the higher layers among all algorithms that have same base layer decisions.
	\label{lem:avoid_skips4}
\end{lemma}
\begin{proof}
No-Pref GroupCast skips the earliest chunks if there are any. Exchange algorithm (algorithm 4) replaces any layers fetched over link 2 by earliest possible. Hence, all chunks fetched using lower priority links are the earliest possible. Therefore, if the ordered set of base layers that are decided to be fetched by link 2 for the Pref GroupCast is $i_1, i_2, \cdots, i_H$ and for any feasible algorithm with same number of layers decided to be fetched by link 2 which are $j_1, j_2, \cdots, j_H$, then $i_k \le j_k$ for  all $k = 1, \cdots, H$.  We know that earlier skips and moving earlier layers to link 2 (less preferable link) provides available bandwidth for more chunks in link 1 since it comes before the deadline of more chunks. This proves the result as in the statement of the lemma since any other feasible algorithm with more number of  layer skips/movements will achieve smaller objective when $\lambda$'s satisfies \eqref{basic_gamma_1}, thus showing that it will not be optimal. 
\end{proof}


Combining these results, the following theorem shows the optimality of the proposed algorithm. 
\begin{theorem}	
	Up to a given enhancement layer
	$M, M \geq 0$, if ${z_{m}^{(u)}(i,j)}^*$ is the size of the $m$th layer fetched by the $u$th use ($m \leq M$) of chunk $i$ that is found by running Avoid-Skips GroupCast algorithm, and ${z_{n}^{(u)}(i,j)}^\prime$ is a size that is found by any other feasible algorithm such that all constraints are satisfied, then the following holds when $\lambda$'s satisfy (\ref{basic_gamma_1}) .%for any $0<\gamma \ll 1$. %and $\sum_{j > k}\gamma^j \sum_i Z_{j,i} \ll \gamma^k  Z_{k,1}$.
	\begin{align}
	& \sum_{i=1}^C\sum_{j=1}^{(i-1)L+s}\sum_{n=0}^{N}\Big(\lambda_n^1{z_n^{(1)}(i,j)}^\prime+\lambda_n^2{z_n^{(2)}(i,j)}^\prime\Big) \\& \leq  \sum_{i=1}^C\sum_{j=1}^{(i-1)L+s}\sum_{n=0}^{N}\Big(\lambda_n^1{z_n^{(1)}(i,j)}^*+\lambda_n^2{z_n^{(2)}(i,j)}^*\Big)
	\label{thm:thm_avoidSkips}
	\end{align}
	In other words, Avoid Skips GroupCast finds the optimal solution to the optimization problem~(\ref{equ:eq1}-\ref{equ:c9eq1}) when $\lambda$'s satisfy (\ref{basic_gamma_1}) and for the Avoid-Skips with two users.
	
	\label{theorem: theorem1}
\end{theorem}
%\vspace{0.5in}
\begin{proof}
Use of  Lemma \ref{lem:avoid_skips} shows that the proposed algorithm is optimal for base layer skips, and use of Lemma \ref{lem:avoid_skips3} shows that the algorithm achieves the minimum number of base layer skips with minimum usage of link 2 (less preferable link).  According to lemma \ref{lem:avoid_skips4}, running Avoid-Skips GroupCast algorithm offers the maximum bandwidth per chunk for $E_1$ layer decisions among all feasible algorithms with same number of skips. Therefore, the bandwidth that is passed to $E_1$ decision is the maximum per chunk. The rest of the algorithm is a running of No-Pref GroupCast for link 1 and a link with the bandwidth being zero all times. No-Pref GroupCast is shown to be optimal in avoiding skips theorem \ref{them:skip1} and optimal in providing more bandwidth to every chunk by skipping the layers of the earliest chunks if there are any \ref{lem:avoid_skips4}. Therefore, No-Pref GroupCast is achieving the optimal decision of the $n^{th}$ layer and passing the optimal bandwidth profile to the $(n+1)^th$ layer. This concludes the proof.
\end{proof}






==> problem.tex <==
\subsection{Skip Based Streaming: Problem Formulation}
\label{sec:problem}

In this section, we describe our cooperative SVC video streaming problem formulation. Let us assume a video divided into $C$ chunks (segments), where every chunk is of length $L$ seconds, is encoded in Base Layer (BL) with rate $r_0$ and $N$ enhancement layers ($E_1, \cdots, E_{N}$) with rates $r_1, \cdots, r_{N}$,  respectively. Note that $Y_n=L*r_n$ is the size of the $n$th layer. $Z_{n,i}$ denotes the size of the $n$th layer that has been fetched. Therefore, if the $n$th layer can be fetched $Z_{n,i}=Y_n$; otherwise $Z_{n,i}=0$. 


%The size of a chunk delivered up to layer $n$ is $X_{i,n}=\sum_{l=0}^n Z_{n,i}$.
%$Y_i$ $\in$ ${\mathcal Y}$, Where  ${\mathcal Y}$ is a set of all possible chunk sizes including 0.
 Let $z_n^{(u)}(i,j)$ be the size of layer $n$ of chunk $i$ fetched through the $u$th contributor at time slot $j$. Let $B^{(u)}(j)$ be the available bandwidth over the $u$th link. Let $S$ be the startup delay. We assume all time units are discrete and the discretization time unit is assumed to be 1 second. %Since the chunk size is $L$ seconds, the buffer occupancy  increases by $L$ seconds when chunk $i$ starts downloading.


%We start by assuming that the decision is taken at the application layer where a layer of a chunk  cannot be split over the two paths (or links). It must be fully downloaded over either of the paths.  In other words, $\left(\sum_{j=1}^{(i-1)L+s} z_n^{(1)}(i,j)\right)\left(\sum_{j=1}^{(i-1)L+s} z_n^{(2)}(i,j)\right) = 0$ for all $n$ and $i$. 


Now, we describe our problem formulation assuming perfect prediction for the whole period of the video (Offline) and infinite buffer size. We will relax these assumption when we describe our online algorithm in section.~\ref{}.

They key objectives of the problem for a given set of weights and/or maximum contribution per contributing user are \emph{(i)} minimization of  the number of skipped chunks, \emph{(ii)} maximization of the average playback rate of the video,  and \emph{(iii)} minimization of  the quality changes between the neighboring chunks to ensure that perceived quality is smooth\footnote{Though we have not considered (iii) explicitly in the problem formulation, we select the algorithm which gives fewer quality variation among the set of optimal solutions.} .


%In order to account for the these objectives, we consider an optimization objective of:
%\begin{equation}
% \sum_{n=0}^{N}\lambda_n\sum_{i=i^\prime}^{C} Z_{n,i}-\sum_{j=j^\prime}^{deadline(C)} \frac{\mu_u}{w_u}B^u(j)-\sum_{j=j^\prime}^{deadline(C)} \frac{\mu_v}{w_v}B^v(j)
% \end{equation}
 
% In the above equation we maximize weighted sum of the chunk layers and we minimize the different link usages based on the provided weights. $w_u$ is the weight of the $u$th LTE link, and $w_v$ is the weight of the $v$th WiFi link. For example if $w_v=\infty$, the minimization term of the bandwidth usage of $v$th link goes to zero which means this link can be used as much as it can provide bandwidth. i.e there is no limit on how much this link can be used. In the other hand if there is a link $u$ such that $w_u=0$, the $u$th link can't be used at all. Finally, $\mu_u$ and $\mu_v$ are weights of the minimization terms of the different links based on how these links were used prior to the current optimization window. In other words, to maintain long term $w_u$ and $w_v$, we need to consider how heavy different links been used prior to the current optimization window.

In order to account for the these objectives, we consider an optimization objective of:
\begin{equation}
 \sum_{u=1}^U\sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C}\sum_{j=1}^{dealine(C)} z_{n}^{(u)}(i,j)
\label{equ:mainObj}
 \end{equation}
 Where user IDs are ordered according to their priority level. For example, if there is a user with unlimited plan, $u=1$ will be assigned to that user.
  
 In the above equation we maximize weighted sum of the chunk layers where
 
The weight choices must satisfy the following two constraints:
\begin{equation}
 \lambda_0^{(1)} > \lambda_0^{(2)} >...> \lambda_0^{(N)}>  \lambda_1^{(1)}......> \lambda_U^{(N)}
 \end{equation}
 , and the following hold through for any user with index $k$, and any users with induces $u > k$, and $u^\prime < k$:
 \begin{align}
 &\lambda_a^{(k)} Y_{a} > \Big(C \cdot \sum_{n=a+1}^{N}\lambda_{n}^{u} Y_n+C \cdot \sum_{n=0}^{N}\lambda_n^{u}Y_n \nonumber \\&+C \cdot \sum_{n=a+1}^{N}\lambda_n^{u^\prime}Y_n\Big)
 %&\lambda_a^{(k)} Y_{a} > \Big(C \cdot \sum_{n=a+1}^{N}\lambda_{n}^{u} Y_n+\sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C} Y_n \nonumber \\&+\sum_{n=a+1}^{N}\lambda_n^{u^\prime}\sum_{i=1}^{C} Y_n\Big)
\end{align}

%\begin{align}
 %&\lambda_a^{(k)} Y_{a} > C \cdot \sum_{n=a+1}^{N}\lambda_{n}^{u} Y_n+{\bf 1}\{u > k\}\cdot \sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C} Y_n \nonumber \\&+{\bf 1}\{u^\prime < k\}\sum_{n=a+1}^{N}\lambda_n^{u}\sum_{i=1}^{C} Y_n
%\end{align}
First, this choice of $\lambda$'s implies that all the higher layers than layer $a$ have lower utility than a chunk at layer $a$ for all $a$. For $a=0$, this implies that all the enhancement layers have less utility than a chunk at the base layer. Thus, the avoidance of skips is the highest priority. The use of $\lambda$ helps in giving higher priority to fetch more chunks up to $n$th layer quality over fetching some at higher quality in the cost of fetching other chunks at quality that is below $n$th layer. In other words, it prioritizes horizontal over vertical scan, and implicitly, this will also reduce un-necessary layer switching. 
Second, it implies that the highest utility is achieved for every layer that can be fetched is when that layer is fetched by the user with the highest priority. This will obey the priority order, and it will not user a lower priority order user to fetch a layer that can be fetched by a higher priority order user.
Note that the system gets a strictly increasing utility depending on the rate it watches the video. The utility function is most often considered to be a concave function. Thus, the rate of increase in the utility decreases with the play-back rate and hence the weights of lower layers are much higher than those of higher layers. 



Since the objective will be constrained to the maximum number of bytes that can be a fetched on each link, the link usage still can enforce the quality to reduce, but that is not part of the objective function, instead we have it as a constraint.

Overall, the multi-path SVC layer scheduling problem with the knowledge of future bandwidth information can be formulated as follows.


\begin{eqnarray}
maximize   \sum_{u=1}^U\sum_{n=0}^{N}\lambda_n^{u}\sum_{i=1}^{C}\sum_{j=1}^{dealine(C)} z_{n}^{(u)}(i,j)%- \lambda \sum_{j=1}^{deadline(C)} B(j)^{(2)}  \Bigg)
 %\sum_{n=0}^{N} \lambda_n \gamma^n \sum_{i=1}^{C}\beta^i B_{n,i}^{(2)}  \Bigg)
\label{equ:eq1}
\end{eqnarray}
\vspace{-.1in}
subject to
%\begin{eqnarray}
%\sum_{j=1}^{(i-1)L+s} z_0^{(2)}(i,j)+z_0^{(1)}(i,j) = Z_{0,i}   \forall i 
%\label{equ:c1eq1}
%\end{eqnarray}
%\vspace{-.1in}
\begin{eqnarray}
\sum_{j=1}^{(i-1)L+s}\sum_{u=1}^Uz_n^{(u)}(i,j) = Z_{n,i}\quad  \forall i,  n 
\label{equ:c2eq1}
\end{eqnarray}
\vspace{-.1in}
\begin{eqnarray}
Z_{n,i}\le \frac{Y_n}{Y_{n-1}}Z_{n-1,i}\quad  \forall i,  n>0 
\label{equ:c2eq11}
\end{eqnarray}
\vspace{-.1in}
\begin{eqnarray}
\sum_{n=0}^N\sum_{i=1}^{C} z_n^{(u)}(i,j)  \leq B^{(u)}(j) \  \   \forall u, \forall j,
\label{equ:c3eq1}
\end{eqnarray}
\vspace{-.1in}
\begin{equation}
\left(\sum_{j=1}^{(i-1)L+s} z_n^{(u)}(i,j)\right)\left(\sum_{j=1}^{(i-1)L+s} z_n^{(u^\prime)}(i,j)\right) = 0\   \forall i, n, u, u^\prime
\label{equ:c5eq1}
\end{equation}
\begin{equation}
\sum_{j=1}^{deadline(C)} z_n^{(u)}(i,j) \leq max^u\   \forall u
\label{equ:c5eq10}
\end{equation}
\vspace{-.1in}
\begin{equation}
z_n^{(u)}(i,j) \geq 0\   \forall u, \forall i 
\label{equ:c55eq1}
\end{equation}
\vspace{-.1in}
\begin{equation}
z_n^{(u)}(i,j)= 0\   \forall \{i: (i-1)L+s > j\}, \forall u
\label{equ:c6eq1}
\end{equation}
\vspace{-.1in}
\begin{equation}
Z_{n,i} \in {\mathcal Z}_n\triangleq \{0, Y_n\} \quad  \forall i, n
\label{equ:c7eq1}
\end{equation}
\vspace{-.2in}
\begin{eqnarray}
\text{Variables:}&& z_n^{(u)}(i,j),  Z_{n,i} \ \ \  \forall   i = 1, \cdots, C, \nonumber \\&& j = 1, \cdots, (C-1)L+s, n = 0, \cdots, N \nonumber
\end{eqnarray}
%We consider 2 scenarios, Multi-Path TCP, and application layer for link-layer assignment. In the second scenario (Application layer), the following constraint is added to the optimization problem (\ref{equ:eq1}-\ref{equ:c7eq1}). The constraint is added to guarantee that a layer can't be split over two links.
%\begin{equation}
%z_n^{(2)}(i,j)*z_n^{(1)}(i,j) = 0\   \forall i = 1, \cdots, C, and \forall j = 1, \cdots, deadline(C)
%\label{equ:c5eq1}
%\end{equation}

In the above formulation, $\lambda$'s are constrained by \eqref{basic_gamma_1}, so we prioritize lower layers compared to higher layers as mentioned earlier. %Further, there is a penalty for the use of link $1$ in the objective function.  %\textcolor{red}{Moreover, we consider different values of $\lambda$. For example, $\gamma^2 < \lambda < \gamma$, so link 1 is guaranteed to be used only to avoid skips, and $\lambda=0$, so link 1 is used only to avoid skips.}%Constraints \eqref{equ:c1eq1} and \eqref{equ:c7eq1} ensure that what is fetched for layer 0 (the base layer) of chunk $i$ over all links and times to be either zero or the based layer quality.
%
Constraints \eqref{equ:c2eq1} and \eqref{equ:c7eq1} ensure that what is fetched for layer $n$ of chunk $i$ over all links and times to be either zero or $Y_n$. The constraint  \eqref{equ:c2eq11} ensures that $n$th layer of any chunk cannot be fetched if the lower layer has not been fetched.
%
\eqref{equ:c3eq1}  imposes the bandwidth constraint of the two links  at each time slot $j$.
%
Constraint \eqref{equ:c5eq1} enforces a layer of a chunk to be fetched only over one of the paths. Constraint \eqref{equ:c55eq1} imposes the non-negativity of the download of a chunk and \eqref{equ:c6eq1} imposes the deadline constraint since chunk $i\in \{1, \cdots, C\}$ cannot be fetched after its deadline ($deadline(i)=(i-1)L+s$). Recall that $s$  is the initial startup delay.



==> skip_optimality.tex <==
\section{Optimality of No Skip Based  Streaming Algorithm}\label{no_skip_apdx}
%\textcolor{red}{I think the this section except the proof should be moved to the main text} 
The following lemma states formally that the No-Skip GroupCast algorithm achieves the minimum stall duration such that all chunks are at least fetched at base layer quality.

\begin{lemma}
If $d^*(i)$ is the stall duration of chunk $i$ that was found using No-Skip GroupCast algorithm such that all chunks can be at least delivered at base layer quality, and $d^\prime(C)$ is the stall duration of chunk $i$ that was found using any other algorithm, then:\\
$$\sum_{i=1}^{C}d^\prime(i) \geq \sum_{i=1}^{C}d^*(i).$$
In other words, No-Skip GroupCast achieves the minimum stall duration such that all chunks are fetched at least at base layer quality.
%The deadline of chunk $i$ that is found by no skip base layer forward algorithm is the maximum deadline such that stall duration up to chunk $i$ playback time is at its minimum.
\end{lemma}
\begin{proof}
The proposed algorithm is a greedy algorithm that only adds to the deadline if there must be a skip due to not enough bandwidth. Further, the algorithm fetches all the chunks at only base layer quality which would have the lowest possible fetching times. Due to this greedy nature, no other algorithm can fetch all the chunks before those obtained by this greedy algorithm. 
\end{proof}

Having shown the minimum stall durations, All proofs for offline skip version applies since the only difference is that the startup delay is chosen such that there will be no skips. 



==> skipperfect.tex <==
\subsection{Efficient Algorithm}\label{skipalgoEqual}
 
%In this section, we consider the case where $m=N$. We will first ignore $D$, by having $D=0$ and then explain the modification step accounting for the cost of the link $1$. Intuitively, based on Lemma\ref{lem_lower_unc}, obtaining the chunk qualities does not depend on $D$. Thus, we will first determine the qualities of the different chunks. Then, based on Lemma 
 
 In this section, we describe our 
 proposed algorithm ``Cooperative SVC Algorithm". First, we will describe our algorithm for the scenario when all users have the same priority level and all have unlimited plan, so every user can be used equally likely to fetch all layers. We call this algorithm ``No preference Cooperative SVC`` (No-Pref SVC). Then, we describe another algorithm for the very interesting case in which some users can only cooperate to avoid skips (fetch BLs only). We call this algorithm ``avoide-skips-Coop SVC``. We will show both proposed algorithms are optimal. Finally, we will propose a heuristic for the more general case in which some users can cooperate up to a certain enhancement layer. 
 
 
 
\subsubsection{No preference Cooperative SVC}\label{skipalgoNoPref}


The algorithm initially finds the cumulative bandwidth of every second $j$ and user $k$ ($r^{(k)}(j)$), line 4). Then, it makes the decisions for the base layer, \ie which chunks to be skipped, and which to be fetched. Moreover, the algorithm decides which user (link) will be used to fetch the base layer of every fetched chunk. The algorithm performs backward scan startng from the deadline of the last chunk (line 7) and checks the possibility of fetching chunks according to the available bandwidth (line 10). Given the decisions of chunks $i+1, \cdots, L$, we wish to decide which of the links should chunk $i$ be fetched at, such that the objective function is maximized without violating deadline, bandwidth, and rate constraints. For all choices of links (users) at which chunk $i$ can be fetched, we compute the residual total bandwidth (sum of the bandwidths of all links) that will remain for the download of the chunks $1, \cdots, i-1$. The link choice that maximizes the residual total bandwidth is chosen to fetch chunk $i$ (Algorithm 2). Note that the algorithm is similar to  dynamic programming, where the algorithm decides the quality at which the chunks will be fetched starting from the last one. The link over which the chunk $i$ is fetched is the one that gives the maximum amount of total available bandwidth over all links before the deadline of chunk numbered $i-1$.  For example, consider that there are only two links, and consider that fetching the $i$-th chunk over the  link 1 results in using  $x$ amount of the bandwidth before the deadline of $i-1$-th chunk while fetching the $i$th chunk over  link 2 results in using  $y$ amount of the bandwidth before the deadline of $i-1$th chunk. Then, the first link will be chosen to fetch the chunk $i$ if $x<y$. 

Once the base layer decision is taken, the algorithm sequentially decides to fetch the enhancement layers. %in a similar fashion.

{\bf Enhancement layer modifications}: The algorithm proceeds in a similar fashion to decide for the next higher layer and so on.  The bandwidth is now modified to be the remaining bandwidth after excluding whatever used to fetch lower layers (line 10, Algorithm 2).  Also note that $n$th layer for a chunk is not fetched if its $(n-1)$th layer was not fetched (line 9, Algorithm \ref{algo:mpsvc}).


%than the remaining size of the $n$th layer is considered to be moved to the next set if it can be fetched over a link in that set before its deadline. Since in this case the moved layer is still less than the required size, the algorithm continue checking the possibility of moving another one with a size equal (or less than if there is no equal) to the remaining size. Therefore, what the algorithm moves to the next set every time a layer can't be fetched is upper bounded by a size of the smallest fetched layer. 


%will move the lowest number of layers from previously fetched chunks to the next set of links such that the $n$th layer can be completely fetched over a link belong to this set. We know that we need $c1*BL+c2*E1+c3*E2+....+c_{n-1}E_{n-1}+c_{n}E_{n}$, and we know how many out of every layer have been fetched for all previous chunks. We sort the fetched layers according to their sizes, we start with the max size one, and check how many out of it can be moved to the next set such that the free space is less than or equal to the $n$th layer size, we proceed to the next highest layer till we see that adding one more of that layer will exceed the  remaining size of the $n$th layer, we fill the remaining from the minimum fetched layer, if all minimum fetched layers are moved we proceed to the next layer in size in order. %and we define the layer with minimum size among all fetched  as $min$th layer, and the one with max size as $max$, then the combination we move is %\sum_{i=1, i \neq m^n c_i 

%The way we find the lowest combination is by dividing the remaining (un-fetched) size of this layer with every layer size, (we find the coefficients $c1,....,c_n$), so


\begin{figure}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:}  $\mathbf{Y}=\{Y_n\forall n\}$, $L$, $s$, $C$, $U$, $\mathbf{B}^{(u)}=\{B^{(u)}(j)\forall j\}$, $u=1, 2,......,U$. 
				\STATE {\bf Output:} $I^{(u)}_{n}$, $u=1,...,U$, $n=0,...,N$: set containing the indices of the chunks that can have their $n$th layer fetched over link $u$.
					
    \STATE  $deadline(i)=(i-1)L+s \quad \forall i$ 
     \STATE  $r^{(u)}(j)=\sum_{j^\prime=1}^{j} B^{(u)}(j^\prime)$, $j=1,....deadline(C)$, $u=1,...., U$
    % \STATE $remainigLayers \leftarrow$ $\mathbf{Y}=\{Y_n\forall n\}$
    \FOR{each layer $n = 0, \cdots, N$}
      
     \STATE $j_{1}=j_{2}=....=j_{U}=deadline(C)$
    %\FOR{$u=1:U$}
     %{\bf j not defined - need efficient loop - should be also outside $n$ loop. }
    % available bandwidth on lte connection up to time $j, \forall j$
    \FOR{$i=C:-1:1$}
    \STATE $j_k =\min(j_k, deadline(i))$, $k$
    	\IF{($n=0$ or $i \in I_{n-1}^{(1)}$ or $i \in I_{n-1}^{(2)})$}
    		\IF{$max(r^{(1)}(j_1),...., r^{(U)}(j_2)) \geq Y_n$}
      			\STATE $[R^{(u)},B2^{(u)}, j2^{(u)}, nf^{(u)}] = backward(i, j_u, \{r^{(u)}(j)\forall j\}, \mathbf{B}^{(u)}, Y_n)$, $u=1, 2,...U$
      		%	\STATE $tmp^{(k)}=0$, $k=1, 2$% {\bf Anis, check $\infty$ or zero, since you will be doing max later. If not fetched and has infinite residual bandwidth, this will be chosen. }
      		%	\FOR{k=1:2}
      		%	\IF{$nf^{(k)}=0$}
      			\STATE $tmp(u)=(1-nf^{(u)})R^{(u)}(deadline(i-1))+\sum_{u^\prime=1, u^\prime \neq u}^{U} r^{(u^\prime)}(deadline(i-1))$, $u=1, 2,...U$
      		%	\ENDIF
      		%	\ENDFOR
      			\STATE $u_1=\arg\max \big(tmp^{(u)\big)}$
      			\IF { $(r^{(u_1)}(deadline(i)) \geq Y_n)$}
      				\STATE $I_n^{(u_1)}=I_n^{(u_1)} \cup i$
      				\STATE $\mathbf{B}^{(u_1)}=B2^{(u_1)}$, $j_{u_1}=j2^{(u_1)}$, $r^{(u_1)} =R^{(u_1)}$
				\STATE $Y_n=0$
      			\ENDIF
			%\ELSE
			%\STATE $Y=move()$
      		\ENDIF
	\ENDIF
      \ENDFOR
     \ENDFOR
    % \ENDFOR
   				\end{algorithmic}
				\caption{No-Pref SVC Algorithm }\label{algo:mpsvc}
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}






\begin{figure}
		%\vspace{-.6in}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $i, j, r, B, Y_n$
					\STATE {\bf Output:} $R$ is the residual cumulative bandwidth at different times after fetching chunk $i$, $B2$ is the residual bandwidth after accounting for fetching of chunk $i$, $j2$ is the index at which chunk $i$ starts being fetched, $nf$ determines whether chunk $i$ can be fetched, 1 if it is can't be fetched. 
    \STATE {\bf Initialization:}
    \STATE $i=C$,  $nf=0$
    \IF{$r < Y_n$}
    	\STATE $nf=1$
	\ELSE
     \WHILE {($Y_n > 0$)}

            \STATE $fetched=min(B(j), Y_n)$ 
            \STATE $B(j)=B(j)-fetched$, $r(j)=r(j)-fetched$, $Y_n(i)=Y_n(i)-fetched$
	   \STATE {\bf if } {$(B(j)=0)$} {\bf then }  $j=j-1$            	
    \STATE $R=r$, $B2=B$, $j2=j$        
\ENDWHILE
\ENDIF
				\end{algorithmic}
				\caption { Backward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}
	
	

{\bf Complexity Analysis}:  The algorithm sequentially decides  each layer one after the other, and thus it is enough to find the complexity of one layer to compute overall algorithm complexity. 
For each layer $n$, the algorithm first finds the cumulative bandwidth of every time slot $j$, $r^{(k)}(j)$ which is linear complexity. Then, it starts from the last chunk, and performs  the backward algorithm on each link at each time. The backward algorithm determines whether the chunk can be fetched in that link and the amount of residual bandwidth. Since the complexity of backward algorithm is linear in $C$, the overall complexity for a layer is $O(C^2)$. Thus, the overall complexity is $O(NC^2)$. 
 
 \begin{remark}
In our algorithm, with the use of $\lambda$, the lower layers have higher priority than the higher layers. 
%
%always prefer pushing {\em all} chunks to $n$th layer quality rather than fetching {\em some} chunks at $(n+1)$th and  {\em some}  others at $(n-1)$th qualities {\bf Vaneet: I re-wrote your statement, please check if it is better now}. 
The algorithm also prefers to utilize the excess bandwidth to fetch the later chunks rather than earlier chunks. Hence, our proposed algorithm reduces the un-necessary quality variation across neighboring chunks. 
\end{remark}
 
 

==> skipperfect_E.tex <==
\subsection{Link Preference ($\gamma^{(m+1)} < \lambda < \gamma^{m}$)}
\label{skipalgoPref}

In this section, we describe our 
 proposed algorithm when one of the links need to be used less than the other one because one could be more expensive or less energy efficient. The algorithm is called ``Multi-Path-Pref SVC Algorithm" (MP-Pref-SVC).
 
 Initially, MP-Pref-SVC algorithm follows the same steps of MP-SVC up to the $m$th layer. Therefore, the fetching policy such that both links are equally likely to be used and maximum number of chunks that can be fetched up to $m$th layer quality level is found. However, up to this point, the decision did not consider minimizing the usage of link 1. To do so, forward algorithm (algorithm 4) is run in order to simulate fetching the layers according to the policy that was found using up to $m$th layer MP-SVC but with prioritizing fetching chunks on link 2. The algorithm starts from the base layer of the first chunk that was decided to be fetched, and checks the possibility of fetching it over link 2 first(lines $12-16$). If $k$th layer of chunk $i$ can't be totally fetched on link 2 before its deadline, it is assigned to link 1(lines $17-21$). Therefore, forward algorithm ensures that chunks can be fetched according to $m$th layer MP-SVC decision with minimum use of link 1.
 
 Since $\lambda > \gamma^{(m+1)} $, all layers starting from $(m+1)$th up to the highest layer can't be fetched on link 1; Otherwise, the objective is minimized instead of being maximized. Therefore MP-SVC still can be run for those layers but considering that the link 1 input bandwidth is only the amount that is needed to satisfy MP-SVC fetching policy up to the $m$th layer.  
 
 

\begin{figure}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE Run MP-SVC algorithm for layers $n=0$ to $m$
				\STATE $B^{(1)}$=forward($C, r^{(1)}, r^{(2)} B^{(1)}, B^{(2)}, Y_{1,...,m}(i), I_{1,...,m}^{(1)}, I_{1,...,m}^{(2)}$)
				\STATE Run MP-SVC algorithm for all layers. i.e $n=0$ to $N$
				   \end{algorithmic}
				\caption{Offline MP-Pref-SVC Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}


 
 \begin{figure}
		%\vspace{-.6in}
		\vspace{-.1in}
		\begin{minipage}{\linewidth}
			\begin{algorithm}[H]
				\small
				\begin{algorithmic}[1]
				\STATE {\bf Input:} $C, r^{(1)}, r^{(2)} B^{(1)}, B^{(2)}, Y_n(i), I_n^{(1)}, I_n^{(2)},\quad n=1,...m$
					\STATE {\bf Output:} $R$ is the residual cumulative bandwidth at different times after fetching chunk $i$, $B2$ is the residual bandwidth after accounting for fetching of chunk $i$, $j2$ is the index at which chunk $i$ starts being fetched, $nf$ determines whether chunk $i$ can be fetched, 1 if it is can't be fetched. 
    \STATE {\bf Initialization:}
    \STATE $i=1$
    \STATE $j_k=1$
    \STATE $n=0$
    \STATE $B^{(k)}_{tmp}=B^{(k)}$, and $r^{(k)}_{tmp}=r^{(k)}$
    \WHILE{$(i \leq C)$}
    	\WHILE{$(n \leq m)$}
	 	\IF{$(i \in I_n^{(1)}$ or $i \in I_n^{(2)})$}
			\IF{($j$ is the first time in which layer $n$ of chunk $i$ is fetched)}
   				\IF{$(r^{(2)}_{tmp}(deadline(i))-r^{(2)}_{tmp}(j2) \geq Y_n(i)$}
   					\IF{$(i \in I_n^{(1)})$}
   						\STATE $I_n^{(2)}=I_n^{(2)} \cup i$
						\STATE $I_n^{(1)}=I_n^{(1)} \ \ i$
					\ENDIF
				\ELSIF{$(r^{(1)}_{tmp}(deadline(i))-r^{(1)}_{tmp}(j1) \geq Y_n(i)$}
					\IF{$(i \in I_n^{(2)})$}
						\STATE $I_n^{(1)}=I_n^{(1)} \cup i$
						\STATE $I_n^{(2)}=I_n^{(2)} \ \ i$
					\ENDIF
				\ENDIF
			\ENDIF
		\ENDIF
				
	   \IF{$(i \in I_n^{(k)})$}
            	\STATE $fetched=min(B^{(k)}_{tmp}(j_k), Y_n(i))$ 
            	\STATE $B^{(k)}_{tmp}(j_k)=B^{(k)}_{tmp}(j_k)-fetched$
		\STATE $r^{(k)}_{tmp}(j_k)=r^{(_k)}_{tmp}(j_k)-fetched$
	%\ELSIF{$(i \in I_n^{(1)})$}
            	%\STATE $fetched=min(B^{(1)}_{tmp}(j1), Y_n(i))$ 
            	%\STATE $B^{(1)}_{tmp}(j1)=B^{(1)}_{tmp}(j1)-fetched$, $r^{(1)}_{tmp}(j1)=r^{(1)}_{tmp}(j1)-fetched$
	\ENDIF
            
            \STATE $Y_n(i)=Y_n(i)-fetched$
	   \STATE {\bf if } {$(B(j_k)=0)$} {\bf then }  $j_k=j_k+1$, $k=1,2$
	     %\STATE {\bf if } {$(B(j1)=0)$} {\bf then }  $j1=j1+1$
	   %\STATE {\bf if } {$(Y_n(i)=0)$} {\bf then }  $n=n+1$
	   \IF{($(Y_n(i)=0)$)}
	   	   \STATE $n=n+1$
		   	\IF{$(n > m)$}
				\STATE $n=0$, $i=i+1$
			\ENDIF
	    \ENDIF
	   %\STATE {\bf if } {$(Y_n(i)=0)$} {\bf then }  $n=n+1$          	
   % \STATE $R=r$, $B2=B$, $j2=j$        
\ENDWHILE
\ENDWHILE
\STATE $B^{(1)}=B^{(1)}-B^{(1)}_{tmp}$
				\end{algorithmic}
				\caption { Forward Algorithm }
			\end{algorithm}
		\end{minipage}
		\vspace{-.2in}
	\end{figure}

Finally, we created MPTCP-Pref-SVC algorithm by aggregating both bandwidth up to the $m$th layer, and then applying modified version of forward algorithm where only the number of bytes that can't be fetched over link 2 are assigned to link 1. Therefore, in MPTCP forward algorithm a layer can be split into two links. i.e, part of it is fetched over one of the links and the remaining still can be fetched over the other link.
	
\subsubsection{Optimality of the MP-Pref-SVC}\label{optim_skip}

Since MP-Pref-SVC runs MP-SVC up to the $m$th layer, we know from section \ref{} that the optimality holds for the fetching policy of layers $1$ to $m$. Moreover, MP-SVC is run again for the layers $n=0$ to $N$, and if both link bandwidths that are passed to MP-SVC after $m$th layer are the optimal, the decisions of all layers must be optimal. Therefore, the only extra thing that needs to be investigated for the MP-Pref-SVC algorithm is the optimality of the $m$th layer forward algorithm. In other words, if $m$th layer forward algorithm finds the minimum link 1 bandwidth that needs to be used such that all decisions up to the $m$th layer are satisfied, then all the lemmas and the main theorem the proves the optimality of MP-SVC are applicable to MP-Pref-SVC, and the optimality of MP-Pref-SVC follows the same proof of the MP-SVC. The following lemma states the optimality of the $m$th layer forward algorithm.

\begin{lemma}%{Theorem}
Forward algorithm guarantees fetching all chunks according MP-SVC decisions up to the $m$th layer with minimum usage of link 1. In other words, the link 1 bandwidth that is found by calling forward algorithm is optimal, and no algorithm can achieve same fetching policy with less usage of link 1. 
\label{lem:mpPref}
\end{lemma}


==> skipwindow.tex <==
%\subsection{Skip Based Streaming: Window-Based Adaptation with Prediction Errors}
\subsection{Online Algorithm: Dealing with Unavailable and Inaccurate BW Prediction}
\label{sec:bw_err}

For the algorithm described in Section \ref{skipalgoEqual}, we assumed that perfect bandwidth prediction, and  client buffer capacity is unlimited. However, practically, the prediction will not be perfect, and the client buffer might be limited. In this section, we will use an online algorithm that will obtain prediction for a window of size $W$ chunks ahead and make decisions based on the prediction. Note that the buffer capacity at the user may be limited, and in that case we consider that $W$ is no more than the buffer capacity since the chunks beyond that will not be fetched in the algorithm. The way we capture the buffer capacity is by assuming that at every re-run of the algorithm (every $\alpha$ seconds), only chunks that are $B_{max}$ ahead of the chunk that is currently being played can be fetched.
%{\bf Vaneet, I tried to say something here, but I am sure this way of describing it is bad. Would you mind re-phrasing it in a better way}
%In fact, with current devices (several Giga Bytes of RAM), the memory is not an issue. Devices can store many chunks ahead but with the concern of the media sources about users fetching many chunks ahead, compete the bandwidth with other users and then do not continue watching, it became necessary to bound the number of ahead chunks that can be fetched at any given time (just in time video
 There are multiple ways to obtain the prediction, including a crowd-sourced method to obtain historical data \cite{Riiser12,GTube}. Another approach may be to use a function of the past data rates obtained as a predictor for the future, an example is to compute the harmonic mean of the past $\beta$ seconds to predict the future bandwidth ~\cite{chen2016msplayer}. The decisions are re-computed for the remaining chunks periodically every $\alpha$ seconds. 


For the prediction window $W$, the algorithm in Section \ref{skipalgoEqual} is run to find the quality using the predicted bandwidth profile, then the $W$ chunks are fetched according to the algorithm decision. At any time slot before next $\alpha$, if there is excess bandwidth (the real bandwidth turns to be higher than the predicted value), this excess is used to fetch what was supposed to be fetched at the later times. However, we do not change the decision which layer of the chunk to be fetched using link 1 or 2. If the bandwidth is lower, then the content to be fetched will be shifted to next time and the content that misses the deadline will no longer be fetched.  If after obtaining the chunks for the entire window $W$, there is  excess bandwidth, and the buffer still allows for more chunks to be fetched, the chunks after the window are fetched at the highest layer.  If the buffer occupancy is lower than a pre-decided threshold $B_{min}$, chunks are fetched at most in base layer, which also includes the fetching of the first few chunks.

==> sysModel.tex <==
\section{System Model}
In this section, we will describe the system model. Fig~\ref{fig : sysModel} show an example describes our model. The system in general consists of $U$ contributors (orthogonal links such as LTE UEs and WiFi access points), a single display, and a controller which can be stand alone, built in the display device, or elected among the users. The UEs have different data plans (\eg 3GB, 6GB, and unlimited). We assume that the users are interested in watching the same video on the same screen. Moreover, we assume the video is SVC encoded into multiple Base layer (BL) and multiple enhancement layers $EL_1,....EL_N$, and we consider two scenarios: the skip based streaming and the no-skip based streaming. For the skip based streaming, the video is played with an initial start-up, (\textit{i.e.,} buffering) delay $s$ and there is a playback deadline for each of the chunks where chunk $i$ need to be downloaded by time $deadline(i)$. Chunks not received by their respective deadlines are skipped. For the no-skip based streaming, it also has a start-up delay. However, if a chunk cannot be downloaded by its deadline, it will not be skipped. Instead, a stall (\textit{i.e.,} re-buffering) will occur, \textit{i.e.,} the video will pause until the chunk is fully downloaded.
In both scenarios, the goal of the scheduling algorithm is to determine up to which layer we need to fetch for each chunk (except for those skipped), such that  the number of stalls or skipped chunks is minimized as the first priority and the overall playback bitrate is maximized with minimum usage of the limited plan devices as the next priority. Further, we need to determine which of the available paths to use to fetch each layer of each chunk that is decided to be downloaded.

Users can cooperate in fetching the video chunks, but they are introducing constraints based on their data plans. For example, Fig~\ref{fig : sysModel} shows an SVC encoded video in 1 BL and 3 ELs, and 4 users. The first user is a WiFi access point which has no download limit, so by default all layers are checked and it can be used  to increase the quality as much as the available bandwidth allows. The second user is LTE user with an unlimited plan and has chosen to contribute as much as the available bandwidth allows. Therefore, the priority level of WiFi1 and LTE1 is same. However, the 3rd user has a limited plan $6GB$, but he/she is willing to contribute to increase the quality of the chunks up to the $EL_1$ quality if both 1st and 2nd users fail to do so due to their available bandwidth. Since the priority level of this user is second, it will not be used if both WiFi1 and LTE1 were able to fetch the BL and $EL_1$ of all the chunks. However, LTE2 is putting extra constraint by introducing the maximum contribution download in bytes. Therefore, this link will not download more than $2GB$ for the whole period of the video. Finally, the last user LTE3 has the minimum plan, the lowest priority level, and is willing to contribute to avoid kips/stalls (fetch BL only) if all other links fail to do so.



\begin{figure}
%\vspace{-.15in}
\centering
\includegraphics[trim=0.3in 0in .1in 0in, clip,  width=.48\textwidth]{./sysFig2.pdf}	
%\vspace{-.7in}
 \vspace{-.3in}
 \centering
 \caption{ System Model.}
 \label{fig : sysModel}
% \vspace{-.1in}
\end{figure}
